Achieving Zero Asymptotic Queueing Delay for Parallel Jobs

Zero queueing delay is highly desirable in large-scale computing systems. Existing work has shown that it can be asymptotically achieved by using the celebrated Power-of-$d$-choices (pod) policy with a probe overhead $d = \omega\left(\frac{\log N}{1-\lambda}\right)$, and it is impossible when $d = O\left(\frac{1}{1-\lambda}\right)$, where $N$ is the number of servers and $\lambda$ is the load of the system. However, these results are based on the model where each job is an indivisible unit, which does not capture the parallel structure of jobs in today's predominant parallel computing paradigm. This paper thus considers a model where each job consists of a batch of parallel tasks. Under this model, we propose a new notion of zero (asymptotic) queueing delay that requires the job delay under a policy to approach the job delay given by the max of its tasks' service times, i.e., the job delay assuming its tasks entered service right upon arrival. This notion quantifies the effect of queueing on a job level for jobs consisting of multiple tasks, and thus deviates from the conventional zero queueing delay for single-task jobs in the literature. We show that zero queueing delay for parallel jobs can be achieved using the batch-filling policy (a variant of the celebrated pod policy) with a probe overhead $d = \omega\left(\frac{1}{(1-\lambda)\log k}\right)$ in the sub-Halfin-Whitt heavy-traffic regime, where $k$ is the number of tasks in each job { and $k$ properly scales with $N$ (the number of servers)}. This result demonstrates that for parallel jobs, zero queueing delay can be achieved with a smaller probe overhead. We also establish an impossibility result: we show that zero queueing delay cannot be achieved if $d = \exp\left({o\left(\frac{\log N}{\log k}\right)}\right)$.

==> Achieving Zero Queueing Delay for Parallel Jobs/achievability.tex <==
{
Before we dive into the proofs of Theorems~\ref{main_theorem_1} and \ref{theorem zero delay}, we first develop more understanding of zero queueing delay on a job level through Lemmas~\ref{lem:max-upper} and \ref{lem:filling}.
Due to the space limit, the proofs of the lemmas are presented in Appendix~\ref{app:lemmas-achievability}.
Then we provide a proof sketch for Theorems~\ref{main_theorem_1} and \ref{theorem zero delay} to outline the main steps.
Detailed proofs of Theorems~\ref{main_theorem_1} and \ref{theorem zero delay} are presented in Sections~\ref{sec:proof-main_theorem_1} and \ref{sec:proof-theorem zero delay}, respectively.
Throughout this section, we assume that the assumptions in Theorem~\ref{main_theorem_1} hold.

\subsubsection*{\textbf{Zero queueing delay and queue lengths}}
Lemma~\ref{lem:max-upper} below gives an upper bound on the expected job delay given the \emph{lengths of the queues} that the tasks of a job are assigned to.
Specifically, suppose the $k$ tasks of a job are sent to $m$ queues ($m\le k$) with queue lengths $n_1,n_2,\dots,n_m$, where the queue lengths have included these newly arrived tasks.  Note that multiple tasks of the job could be sent to the same queue, but to compute the job delay, we only need to consider the last task of the job in that queue.  Let $Y_i$ with $1\le i\le m$ denote the delay of the last task of the job in queue $i$.  Then the job delay can be written as $\max\left\{Y_1,\cdots,Y_m\right\}$.  Lemma~\ref{lem:max-upper} gives an upper bound on $\mathbb{E}[\max\left\{Y_1,\cdots,Y_m\right\}]$.
\begin{lemma}\label{lem:max-upper}
Consider $m$ independent random variables $Y_1,\cdots,Y_m$ with $m\le k$, where each $Y_i$ ($1\le i\le m)$ is the sum of $n_i$ i.i.d.\ random variables that follow the exponential distribution with rate $1$.  In the asymptotic regime that $k$ goes to infinity, if $\max\left\{n_1,\cdots,n_m\right\}=o(\log k)$, then
$$
\mathbb{E}[\max\left\{Y_1,\cdots,Y_m\right\}] \leq \ln k + o(\ln k).
$$
\end{lemma}

The upper bound in Lemma~\ref{lem:max-upper} implies that a sufficient condition for this job to have zero queueing delay is that the lengths of the queues that its tasks are assigned to are of order $o(\log k)$.  As we pointed out earlier, this is different from the single-task job model since here zero queueing delay on a job level allows non-zero queueing delay for each of the tasks.



\subsubsection*{\textbf{Zero queueing delay and states}}
Lemma~\ref{lem:filling} below establishes a condition on the \emph{state seen by a job arrival} for all of its tasks to be assigned to queues of length $o(\log k)$ with high probability, which is a sufficient condition for the job to have zero queueing delay by Lemma~\ref{lem:max-upper}. Specifically, we consider the event that all the $k$ tasks of an incoming job are assigned to queueing positions below some threshold value $\ell$, and let this event be denoted by $\mathrm{FILL}_{\ell}$.  Lemma~\ref{lem:filling} shows that $\mathrm{FILL}_{\ell}$ happens with high probability given a proper condition on the state $\bm{s}$ for several values of interest for $\ell$.  Note that if we take $\ell = h$, which is $o(\log k)$, then $\mathrm{FILL}_{\ell}$ leads to zero queueing delay.  But Lemma~\ref{lem:filling} is more general in the sense that it allows other values for $\ell$, which is essential for other parts of the proofs including proving a state-space collapse result (Lemma~\ref{lem:ssc}) and bounding the dropping probability (Theorem~\ref{theorem zero delay}).
\begin{lemma}[Filling Probability]\label{lem:filling}
Under the assumptions of Theorem~\ref{main_theorem_1}, given that the system is in a state $\bm{s}$ such that
\begin{equation}\label{eq:cond-filling}
\sum_{i=1}^{\ell} s_i \leq \ell\left(1 - \frac{1}{4}\beta N^{-\alpha}\right),
\end{equation}
the probability of the event $\mathrm{FILL}_{\ell}$ for any $\ell\in\{h-1,h,b\}$ can be bounded as $\Pr\left\{\mathrm{FILL}_{\ell}\right\} \geq 1 - \frac{1}{N}$ when $N$ is sufficiently large.
\end{lemma}

Here we provide an intuitive explanation for the condition \eqref{eq:cond-filling} when $\ell = h$. When a job arrives and sees state $\bm{s}$, if we choose one queue uniformly at random from all the queues, then the probability for the chosen queue to have a length of $i$ is $s_i-s_{i+1}$.  So the expected number of spaces below position $h$ in the chosen queue is $\sum_{i=0}^{h} (h-i)(s_i-s_{i+1})=h-\sum_{i=1}^{h} s_i$.  
The batch-filling policy samples $kd$ queues.  Thus the total expected number of spaces below position $h$ in the $kd$ sampled queues is $kd\left(h-\sum_{i=1}^{h} s_i\right)$.  To fit all the $k$ tasks of the incoming job to positions below $h$, we need $k\le kd\left(h-\sum_{i=1}^h s_i\right)$, which becomes the following condition when $d \geq\frac{8}{(1-\lambda)h}=\frac{8N^{\alpha}}{\beta h}$ as required in Theorem~\ref{main_theorem_1}:
\begin{equation*}
\sum_{i=1}^h s_i \leq h\left(1 - \frac{1}{8}\beta N^{-\alpha}\right).
\end{equation*}
We strengthen this requirement to the condition $\sum_{i=1}^h s_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)$ to obtain a high-probability guarantee using concentration bounds based on Hoeffding's results on sampling without replacement \cite[Theorem~4]{Hoe_63}.


\subsubsection*{\textbf{Proof sketch for Theorems~\ref{main_theorem_1} and \ref{theorem zero delay}}}
We start by setting the goal to be proving the zero queueing delay result in Theorem~\ref{theorem zero delay}, and we will see how Theorem~\ref{main_theorem_1} emerges as an essential characterization of the system that is needed for Theorem~\ref{theorem zero delay}.

Considering the condition in Lemma~\ref{lem:filling} on the system state, we upper bound the steady-state job delay $T$ in the following way:
\begin{align}
\mathbb{E}[T] &\leq \mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right]\label{eq:T-upper-1}\\ 
&\mspace{21mu}+ \mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i > h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right]\cdot\Pr\left\{\sum_{i=1}^h S_i > h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\},\label{eq:T-upper-2}
\end{align}
where we have used the fact that $\Pr\mspace{-3mu}\left\{\mspace{-3mu}\sum_{i=1}^h S_i \le h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}\le 1$.  We can easily bound the first summand \eqref{eq:T-upper-1} using Lemma~\ref{lem:filling} since this is the case where all the tasks of an incoming jobs are sent to queues with lengths no larger than $h$, which satisfies $h=o(\log k)$ and thus results in zero queueing delay.

We now focus on bounding the second summand \eqref{eq:T-upper-2}, for which it suffices to show that the probability $\Pr\left\{\sum_{i=1}^h S_i > h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}$ is small enough.  By the Markov inequality,
\begin{align*}
\Pr\left\{\sum_{i=1}^h S_i > h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}
\le\frac{\mathbb{E}\left[\max\left\{\sum_{i=1}^b S_i - h\left(1 - \frac{1}{2}\beta N^{-\alpha}\right), 0\right\}\right]}{\frac{1}{4}\beta N^{-\alpha}}.
\end{align*}
It then boils down to bounding $\mathbb{E}\left[\max\left\{\sum_{i=1}^b S_i - h\left(1 - \frac{1}{2}\beta N^{-\alpha}\right), 0\right\}\right]$, which is what Theorem~\ref{main_theorem_1} achieves.


To prove Theorem~\ref{main_theorem_1}, we follow the general framework of Stein's method (see, e.g., \cite{b14,LiuYin_20}).  The main idea is to couple our Markov chain $\left\{\bm{S}(t) \colon t \geq 0\right\}$ with an auxiliary process that is easier to analyze, and bound their difference through generator approximation.  In particular, we compare the dynamics of $\sum_{i=1}^b S_i(t)$ with a continuous function $x(t)$ given by the following simple fluid model as our auxiliary process:
\begin{equation*}
\dot{x}(t) =(-\delta)\mathds{1}_{\{x>0\}},
\end{equation*}
where $\delta$ is a properly chosen parameter that reflects the drift of $\sum_{i=1}^b S_i(t)$.
We reiterate that a key in our analysis is a novel state-space collapse result (Lemma~\ref{lem:ssc}) that we establish, which characterizes how balanced the queues are from a job's point of view.

Combining the arguments above for bounding \eqref{eq:T-upper-1} and \eqref{eq:T-upper-2}, we can conclude that the steady-state job delay $\expect[T]$ achieves zero queueing delay.
}



==> Achieving Zero Queueing Delay for Parallel Jobs/proof-lem_filling.tex <==
\renewcommand{\thmnamerestated}{Lemma~\ref{lem:filling} (Filling Probability) [Restated]}
\newtheorem*{thmrestatedfilling}{\thmnamerestated}{\bfseries}{\itshape}
\begin{thmrestatedfilling}
Under the assumptions of Theorem~\ref{main_theorem_1}, given that the system is in a state $\bm{s}$ such that
\begin{equation}%\label{eq:cond-filling}
\sum_{i=1}^{\ell} s_i \leq \ell\left(1 - \frac{1}{4}\beta N^{-\alpha}\right),
\end{equation}
the probability of the event $\mathrm{FILL}_{\ell}$ for any $\ell\in\{h-1,h,b\}$ can be bounded as $\Pr\left\{\mathrm{FILL}_{\ell}\right\} \geq 1 - \frac{1}{N}$ when $N$ is sufficiently large.
\end{thmrestatedfilling}


\begin{proof}
Assume that a job arrival sees a state $\bm{S}=\bm{s}$ that satisfies 
\begin{equation*}
\sum_{i=1}^{\ell} s_i \leq \ell\left(1 - \frac{1}{4}\beta N^{-\alpha}\right).
\end{equation*}
We focus on the the number of spaces below the threshold $\ell$ in the sampled queues, denoted by $N_{\ell}$. Then $N_{\ell}$ is the maximum number of tasks that can be put into these queues such that all of these tasks are at queueing positions below $\ell$. Therefore, 
$$
\Pr\left\{\mathrm{FILL}_{\ell}\right\} = \Pr\left\{N_{\ell} \geq k\right\} \geq 1 - \Pr\left\{N_{\ell} \leq k\right\}.
$$

\begin{sloppypar}
Now we bound $\Pr\left\{N_{\ell} \leq k\right\}$.  We can think of the sampling process of batch-filling as sampling $kd$ queues one by one without replacement.  Let $X_1,X_2,\cdots,X_{kd}$ be the numbers of spaces below $\ell$ in the $1$st, $2$nd, \dots, $kd$th sampled queues, respectively.  Then $N_{\ell}=X_1+\dots+X_{kd}$.  It is not hard to see that for each of the sampled queue and each integer $x$ with $1 \leq x \leq \ell$,  
\begin{equation*}
\Pr\{X_i=x\}=s_{\ell-x}-s_{\ell-x+1},
\end{equation*}
and $\Pr\{X_i=0\}=s_{\ell}$.
\end{sloppypar}

\begin{sloppypar}
Note that since we sample without replacement, $X_1,X_2,\dots,X_{kd}$ are not independent.  But we can still derive concentration bounds using a result of Hoeffding \cite[Theorem~4]{Hoe_63}.  By this result, we have $\expect\left[f\left(\sum_{i=1}^{kd}X_i\right)\right]\le \expect\left[f\left(\sum_{i=1}^{kd}Y_i\right)\right]$ for any continuous and convex function $f(\cdot)$, where $Y_1,Y_2,\dots,Y_{kd}$ are i.i.d.\ and follow the same distribution as $X_1$. We take the function $f(\cdot)$ to be $f(x)=e^{-tx}$ with $t>0$.  Then
\begin{align*}
&\mspace{23mu}\Pr\left\{N_{\ell} \leq k\right\}\\
&= \Pr\left\{e^{-tN_{\ell}} \geq e^{-tk}\right\} \\
&\leq e^{tk}\prod_{i=1}^{kd} \mathbb{E}\left[e^{-tY_i}\right] \\
&= e^{tk}\prod_{i=1}^{kd}\left(1 - \sum_{j=1}^{\ell}\left(s_{\ell -j}-s_{\ell-j+1}\right)\left(1 - e^{-tj}\right)\right).
\end{align*}
Since $1-x\le e^{-x}$ for each $x\ge 0$, this can be further bounded as
\begin{align}
&\mspace{23mu}\Pr\left\{N_{\ell} \leq k\right\}\nonumber\\
&\le \exp\left(tk - kd\sum_{j=1}^{\ell} \left(s_{\ell-j}-s_{\ell-j+1}\right)\left(1-e^{-tj}\right)\right)\nonumber\\
&\le \exp\left(tk + kd\sum_{j=1}^{\ell} \left(s_{j - 1} - s_j\right)\left(e^{-t(\ell - j + 1)} - 1\right)\right).\label{lemma2:1}
\end{align}
Rearranging the terms in the sum in \eqref{lemma2:1}, we get
\begin{align}
&\mspace{23mu}\sum_{j=1}^{\ell} \left(s_{j - 1} - s_j\right)\left(e^{-t(\ell - j + 1)} - 1\right)\nonumber\\
&= \left(e^{-t\ell} - 1\right) + \left(e^{t}-1\right)\sum_{j=1}^{\ell} s_je^{-t(\ell-j+1)}.\label{lemma2:2}
\end{align}
Since $1 \geq s_1 \geq \cdots s_{\ell}$ and we have assumed that $\sum_{j = 1}^{\ell} s_j \leq \ell\left(1 - \frac{1}{4}\beta N^{-\alpha})\right)$, \eqref{lemma2:2} is maximized when 
$$
s_1 = s_2 = \cdots = s_{\ell} = 1 - \frac{1}{4}\beta N^{-\alpha}. 
$$
Therefore, the upper bound becomes
$$
\Pr\left\{N_{\ell}\le k\right\} \leq \exp\left(tk + kd\left(e^{-t\ell} - 1\right)\frac{1}{4}\beta N^{-\alpha}\right).
$$


Now we apply the condition that $d \geq \frac{8N^{\alpha}}{\beta h}$ and let $t = \frac{\ln(2\ell) - \ln h}{\ell}$.  Then
\begin{align*}
&\mspace{23mu}\Pr\left\{N_{\ell} \leq k\right\}\\
&\le \exp\left(tk + \frac{2k}{h}\left(e^{-t\ell} - 1\right)\right)\\
&= \exp\left(\frac{k}{h}\left(\frac{h}{\ell}\left(\ln(2\ell) - \ln h\right)+\frac{h}{\ell}-2\right)\right).
\end{align*}
Recall the we have assumed that $\frac{k}{h} = \omega(\log N)$ and $h=\omega(1)$.  Then it can be verified that with a sufficiently large $N$, $\frac{h}{\ell}\left(\ln(2\ell) - \ln h\right)+\frac{h}{\ell}+2N^{-0.5}-2$ is smaller than a negative constant for all $\ell\in\{h-1,h,b\}$.  Thus
$$
\Pr\left\{N_{\ell} \leq k\right\} \leq \exp(-\omega(\log N)) \leq \frac{1}{N}.
$$
As a result,
$$
\Pr\left\{\mathrm{FILL}_{\ell}\right\}\ge 1-\Pr\{N_{\ell}\le k\} \geq 1 - \frac{1}{N},
$$
which completes the proof. 
\end{sloppypar}
\end{proof}


==> Achieving Zero Queueing Delay for Parallel Jobs/proof-lem_max-upper.tex <==
\renewcommand{\thmnamerestated}{Lemma~\ref{lem:max-upper} [Restated]}
\newtheorem*{thmrestatedmax}{\thmnamerestated}{\bfseries}{\itshape}
\begin{thmrestatedmax}
Consider $m$ independent random variables $Y_1,\cdots,Y_m$ with $m\le k$, where each $Y_i$ ($1\le i\le m)$ is the sum of $n_i$ i.i.d.\ random variables that follow the exponential distribution with rate $1$.  In the asymptotic regime that $k$ goes to infinity, if $\max\left\{n_1,\cdots,n_m\right\}=o(\log k)$, then
$$
\mathbb{E}[\max\left\{Y_1,\cdots,Y_m\right\}] \leq \ln k + o(\ln k).
$$
\end{thmrestatedmax}

\begin{proof}
The general proof idea is folklore, but here we derive the exact bounds for our purpose.
Let $M_{X}(s)$ be the moment generating function of a random variable $X$. By assumption, $Y_i = \sum_{j=1}^{n_i} X_{i,j}$, and $X_{i,j}, 1 \leq i \leq m, 1 \leq j \leq n_i$ are all independent and exponentially distributed with mean $1$. Therefore, for any $1 \leq i \leq m, 1 \leq j \leq n_i$ and any $s$ with $0<s<1$,
$$
\begin{aligned}
M_{X_{i,j}}(s) &= \mathbb{E}\left[e^{sX_{i,j}}\right] = \frac{1}{1 - s}, \\
M_{Y_i}(s) &= \mathbb{E}\left[e^{sY_i}\right]=\left(\frac{1}{1 - s}\right)^{n_i}.
\end{aligned}
$$


Let $q = \max\left\{n_1,\cdots,n_m\right\}$. It holds that for any $s$ with $0<s<1$, 
\begin{align}
\exp\left(s\mathbb{E}\left[\max_{j=1}^m Y_j\right]\right) &\leq \mathbb{E}\left[\exp(s\max_{j=1}^m Y_j)\right]\label{eq:jensen}\\
&= \mathbb{E}\left[\max_{j=1}^m \exp(sY_j)\right] \\
&\leq \sum_{j=1}^m \mathbb{E}\left[\exp(sY_j)\right]\label{eq:max-sum}\\
&\leq m\left(\frac{1}{1-s}\right)^q,
\end{align}
where \eqref{eq:jensen} is due to Jensen's inequality and \eqref{eq:max-sum} is true since the maximum is upper bounded by the sum. As a result,
\begin{align}
\mathbb{E}\left[\max_{j=1}^m Y_j\right] &\leq \frac{\ln m}{s} + q \cdot \frac{-\ln(1-s)}{s}\\
& \leq \frac{\ln k}{s} + q \cdot \frac{-\ln(1-s)}{s},\label{eq:upper}
\end{align}
where we have used the assumption that $m\le k$.
Since we assume that $q = o(\log k)$, we can write $q$ as $q = \ell(k)\ln k$ where $\ell(k) \to 0^+$ as $k \to \infty$. Let $s = 1 - \ell(k)$ in \eqref{eq:upper}, then
\begin{align}
\mathbb{E}\left[\max_{j=1}^m Y_j\right] &\leq \frac{\ln k}{1 - \ell(k)}\left(1 - \ell(k)\ln\ell(k)\right)\\
&=(\ln k)\left(1+\frac{\ell(k)}{1-\ell(k)}\right)\left(1 - \ell(k)\ln\ell(k)\right).
\end{align}
Note that $\lim_{k \to \infty} \ell(k)\ln\ell(k) = 0$.  Then as $k \to \infty$,
$$
\mathbb{E}\left[\max_{j=1}^m Y_j\right] \leq (\ln k)(1 + o(1)),
$$
which completes the proof. 
\end{proof}

==> Achieving Zero Queueing Delay for Parallel Jobs/proof-lem_ssc.tex <==
Our proof of Lemma~\ref{lem:ssc} relies on Lemma~\ref{lem:tail} below. 
Lemma~\ref{lem:tail} slightly generalizes the well-known Lyapunov-based tail bounds (see, e.g., \cite{b4}, \cite{b5} and \cite{b6}) in that it allows different drift bounds depending on whether a state $\bm{s}$ is in a set $\mathcal{E}$ or not.  In our proof of Lemma~\ref{lem:ssc}, we only need to let $\mathcal{E}$ be the whole state space.  But this generalization will be needed in the proof of impossibility results in Section~\ref{sec:impossibility}.  We omit the proof of Lemma~\ref{lem:tail} since it only needs minor modification to the arguments used in proving the well-known existing bounds.

\begin{lemma}\label{lem:tail}
Consider a continuous time Markov chain $\left\{\bm{S}(t):t\ge 0\right\}$ with a finite state space $\mathcal{S}$ and a unique stationary distribution $\pi$.  For a Lyapunov function $V: \mathcal{S} \rightarrow [0,+\infty)$, define the drift of $V$ at a state $\bm{s} \in \mathcal{S}$ as 
$$
\Delta V(\bm{s}) = \sum_{\bm{s}' \in \mathcal{S}, \bm{s} \not = \bm{s}'} r_{\bm{s} \to \bm{s}'}(V(\bm{s}') - V(\bm{s})),
$$
where $r_{\bm{s} \to \bm{s}'}$ is the transition rate from state $\bm{s}$ to $\bm{s}'$.  Suppose that
$$
\begin{aligned}
\nu_{\mathrm{max}} &:= \sup_{\bm{s},\bm{s}' \in \mathcal{S}:r_{\bm{s} \to \bm{s}'} > 0} |V(\bm{s}) - V(\bm{s}')| < \infty \\
f_{\mathrm{max}} &:= \max\left\{0,\sup_{\bm{s} \in \mathcal{S}} \sum_{\bm{s}':V(\bm{s}') > V(\bm{s})} r_{\bm{s} \to \bm{s}'}\left(V(\bm{s}') - V(\bm{s})\right)\right\} < \infty.
\end{aligned}
$$
Then if there is a set $\mathcal{E}$ with $B > 0,\gamma > 0, \delta \geq 0$ such that 
\begin{itemize}
\item $\Delta V(\bm{s}) \leq -\gamma$ when $V(\bm{s}) \geq B$ and $\bm{s} \in \mathcal{E}$,
\item $\Delta V(\bm{s}) \leq \delta$ when $V(\bm{s}) \geq B$ and $\bm{s} \not \in \mathcal{E}$,
\end{itemize}
it holds that for all $j \in \mathbb{N}$,
$$
\Pr\left\{V(\bm{s}) \geq B + 2 \nu_{\mathrm{max}}j\right\} \leq \left(\frac{f_{\mathrm{max}}}{f_{\mathrm{max}} + \gamma}\right)^j + \left(\frac{\delta}{\gamma} + 1\right)\Pr\left\{s \not \in \mathcal{E}\right\}.
$$
\end{lemma}

Now we are ready to present to proof of Lemma~\ref{lem:ssc}.
\renewcommand{\thmnamerestated}{Lemma~\ref{lem:ssc} (State-Space Collapse) [Restated]}
\newtheorem*{thmrestatedssc}{\thmnamerestated}{\bfseries}{\itshape}
\begin{thmrestatedssc}
Under the assumption of Theorem \ref{main_theorem_1}, consider the following Lyapunov function:
$$
V(\bm{s}) = \min\left\{\frac{1}{h - 1}\sum_{i=h}^b s_i, b\left(\left(1 - \frac{1}{2}\beta N^{-\alpha}\right) - \frac{1}{h-1}\sum_{i=1}^{h - 1} s_i\right)^+\right\},
$$
where the superscript $^+$ denotes the function $x^+=\max\{x,0\}$.
Let $B = \frac{b - h + 1}{h - 1}\left(\beta N^{-\alpha} + \frac{\log N}{\sqrt{N}}\right)$. Then for any state $\bm{s}$ such that $V(\bm{s}) > B$, its Lyapunov drift can be upper bounded as follows
$$
\Delta V(\bm{s}) = GV(\bm{s}) \leq -\frac{b}{\sqrt{N}}.
$$
Consequently, when $N$ is sufficiently large,
\begin{align*}
\Pr\left\{V(\bm{S}) > B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}\right\}\le e^{-\frac{1}{2}\log^2 N}.
\end{align*}
\end{thmrestatedssc}

\begin{proof}
Consider the Lyapunov function in the lemma, i.e.,
$$
V(\bm{s}) = \min\left\{\frac{1}{h - 1}\sum_{i=h}^b s_i, b\left(\left(1 - \frac{1}{2}\beta N^{-\alpha}\right) - \frac{1}{h-1}\sum_{i=1}^{h - 1} s_i\right)^+\right\}.
$$

We will refer to the first term and second term in the minimum as $\terml$ and $\termr$, respectively.
Let $B = \frac{b - h + 1}{h - 1}\left(\beta N^{-\alpha} + \frac{\log N}{\sqrt{N}}\right)$ and suppose $V(\bm{s}) > B$.  Recall that the drift of $V$ is given by
\begin{equation*}
\Delta V(\bm{s}) = GV(\bm{s}) = \sum_{\bm{s}' \in \mathcal{S}, \bm{s} \not = \bm{s}'} r_{\bm{s} \to \bm{s}'}(V(\bm{s}') - V(\bm{s})),
\end{equation*}
where $r_{\bm{s} \to \bm{s}'}$ is the transition rate from state $\bm{s}$ to $\bm{s}'$. Let $e_i = \left(0,\cdots,0,\frac{1}{N},0,\cdots,0\right)$ be a vector of length $b$ whose $i$th entry is $\frac{1}{N}$ and all the other entries are zero.  
We divide the discussion into two cases.

\noindent\textbf{Case 1:} $\terml\le \termr$.  In this case $V(\bm{s})=\terml$.  When the state transition is due to a task departure from a queue of length $i$, which has a rate of $N\left(s_{i}-s_{i+1}\right)$, then
\begin{equation*}
V(\bm{s} - e_i) =
\begin{cases}
V(\bm{s}), &\text{ if }1\le i<h,\\
 V(\bm{s}) - \frac{1}{N(h - 1)}, &\text{ if } h\le i\le b.
\end{cases}
\end{equation*}
Now consider the state transition due to a job arrival.  Let $a_i$ be the queueing position that task $i$ is assigned to.  Then the next state can be written as 
$$
\bm{s} + e_{a_1} + \cdots + e_{a_k}.
$$
Note that when the event $\mathrm{FILL}_{h-1}$ happens, the dispatcher puts all $k$ tasks to positions below threshold $h - 1$. Then under $\mathrm{FILL}_{h-1}$, $s_i$ does not change for $i\ge h$, which implies that
$$
V(\bm{s} + e_{a_1} + \cdots + e_{a_k}) = V(\bm{s}).
$$
We can show that $\Pr\left\{\mathrm{FILL}_{h - 1}\right\} \geq 1 - \frac{1}{N}$ using Lemma~\ref{lem:filling} since $\termr\ge \terml > B >0$.  Otherwise, i.e., when $\mathrm{FILL}_{h-1}$ is not true, it is easy to see that
\begin{equation*}
V(\bm{s} + e_{a_1} + \cdots + e_{a_k})\le V(\bm{s})+\frac{k}{N(h-1)}.
\end{equation*}

Therefore,
\begin{align*}
\Delta V(\bm{s}) &\leq \sum_{i=1}^b N(s_{i} - s_{i + 1})\left(V(\bm{s} - e_i) - V(\bm{s})\right)+\frac{N\lambda}{k}\frac{1}{N}\frac{k}{N(h - 1)}\\
&= \frac{1}{N(h-1)}-\frac{s_h}{h - 1}\\
&\le \frac{1}{N(h-1)}-\frac{1}{h - 1}\frac{1}{b-h+1}\sum_{i=h}^bs_i.
%&\overset{a}{\leq} \frac{-1}{h-1}\left(\beta N^{-\alpha} - \frac{1}{N}+\frac{\log N }{\sqrt{N}}\right) \\
%&\leq -\frac{b}{\sqrt{N}}.
\end{align*}
By the assumption that $\terml>B$, we have
\begin{align}
\frac{1}{b-h+1}\sum_{i=h}^bs_i &\ge \frac{h-1}{b-h+1}B=\beta N^{-\alpha}+\frac{\log N}{\sqrt{N}}.\nonumber
\end{align}
Inserting this back to the upper bound on $\Delta V(\bm{s})$ gives
\begin{align*}
\Delta V(\bm{s})&\le -\frac{1}{h-1}\left(-\frac{1}{N}+\beta N^{-\alpha}+\frac{\log N}{\sqrt{N}}\right).
\end{align*}
Since $\frac{\beta N^{-\alpha}}{h-1}\ge \frac{N^{-\alpha}}{k}\ge \frac{b}{\sqrt{N}}$ and $\frac{\log N}{\sqrt{N}}\ge \frac{1}{N}$ when $N$ is sufficiently large, this upper bound becomes
\begin{equation*}
\Delta V(\bm{s})\le -\frac{b}{\sqrt{N}}.
\end{equation*}



\noindent\textbf{Case 2:} $\terml > \termr$. In this case $V(\bm{s})=\termr$. Similarly, a task departs from a queue of length $i$ at a rate of $N(s_i-s_{i+1})$.  The change in $V(\bm{s})$ can be bounded as
$$
V(\bm{s} - e_i)-V(\bm{s})\le
\begin{cases}
\frac{b}{N(h-1)}, & \text{ if }1\le i < h,\\
0, \text{ if } h\le i \le b.
\end{cases}
$$
When a job arrives, under the event $\mathrm{FILL}_{h - 1}$,
\begin{equation*}
V(\bm{s} + e_{a_1} + \cdots + e_{a_k})= V(\bm{s})-\frac{kb}{N(h-1)},
\end{equation*}
where we have used the fact that $\termr > B$.  Again, $\Pr\left\{\mathrm{FILL}_{h - 1}\right\} \geq 1 - \frac{1}{N}$ by Lemma~\ref{lem:filling}.  Otherwise, i.e., when $\mathrm{FILL}_{h - 1}$ is not true, $V(\bm{s} + e_{a_1} + \cdots + e_{a_k})\le V(\bm{s})$.

Therefore,
\begin{align}
\Delta V(\bm{s}) &\leq 
\sum_{i=1}^b N(s_{i} - s_{i + 1})\left(V(\bm{s} - e_i) - V(\bm{s})\right)%\nonumber\\
%&\mspace{23mu}
+\frac{N\lambda}{k}\left(1-\frac{1}{N}\right)\left(-\frac{kb}{N(h-1)}\right)\nonumber\\
&\leq \frac{b}{h-1}\left(s_1-s_h\right)-\frac{b}{h-1}\left(1-\frac{1}{N}\right)\left(1 - \beta N^{-\alpha}\right)\nonumber\\
&\leq \frac{b}{h-1}\left(1 - \left(\beta N^{-\alpha} + \frac{\log N}{\sqrt{N}}\right)-\left(1 - \frac{1}{N}\right)\left(1 - \beta N^{-\alpha}\right)\right),\label{eq:sbounds}\\
&=\frac{b}{h-1}\left(-\frac{\log N}{\sqrt{N}}+ \frac{1}{N}\left(1-\beta N^{-\alpha}\right)\right)\nonumber\\
&\leq -\frac{b}{h-1}\frac{\log N -\frac{1}{\sqrt{N}}}{\sqrt{N}},\nonumber
\end{align}
where \eqref{eq:sbounds} is due to the fact that $s_1\le 1$ and the fact that $s_h\ge \beta N^{-\alpha} + \frac{\log N}{\sqrt{N}}$ following similar arguments as those in Case 1 noting that $\terml > \termr > B$.  When $N$ is sufficiently large, this upper bound becomes
\begin{equation*}
\Delta V(\bm{s})\le -\frac{b}{\sqrt{N}},
\end{equation*}
which completes the proof of the drift bound in Lemma~\ref{lem:ssc}.


For this Lyapunov function $V$, under the notation in Lemma~\ref{lem:tail}, we have that $\nu_{\mathrm{max}} \leq \frac{kb}{N(h-1)}$ and $f_{\mathrm{max}} \leq \frac{b}{h-1}$.  Let $\mathcal{E} = \mathcal{S}$ and $j = \sqrt{N}\log^2 N$.  Then by Lemma~\ref{lem:tail}, the drift bound implies that
\begin{align*}
&\mspace{21mu}\Pr\left\{V(\bm{S}) > B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}\right\}\\
&=\Pr\left\{V(\bm{S}) > B + \frac{2kb}{(h-1)N}j\right\}\\
&\leq \left(1 + \frac{h-1}{\sqrt{N}}\right)^{-j} \\
&\leq \left(\left(1 + \frac{1}{\sqrt{N}}\right)^{\sqrt{N} + 1}\right)^{-\frac{1}{\sqrt{N}+1}\sqrt{N}\log^2 N} \\
&\leq e^{-\frac{1}{2}\log^2 N},
\end{align*}
where the last inequality holds when $N$ is sufficiently large.  This completes the proof.
\end{proof}

==> Achieving Zero Queueing Delay for Parallel Jobs/proof-main_theorem_1.tex <==
\begin{proof}
As explained in the proof sketch, we compare our system with the following fluid model:
\begin{equation}\label{eq:fluid}
\dot{x}(t) =(-\delta)\mathds{1}_{\{x>0\}},
\end{equation}
where $x(t)$ is continuous and $\delta=\frac{(k+1)\log N}{\sqrt{N}}$.  
{When viewed as a continuous-time Markov chain, this fluid model (with a possibly random initial state) can be described by its generator \cite{EthKur_86}, denoted as $\overline{G}$ and given by}
\begin{equation*}
\overline{G}g(x)=g'(x)\cdot(-\delta)\mathds{1}_{\{x>0\}}
\end{equation*}
for any differentiable function $g$. Recall that we will compare the dynamics of $\sum_{i=1}^b S_i(t)$ in our load-balancing system with $x(t)$.

\begin{sloppypar}
The quantity of interest in Theorem~\ref{main_theorem_1} is $\expect\left[\max\left\{\sum_{i=1}^b S_i - \eta, 0\right\}\right]$, where we have used the notation $\eta=h\left(1 - \frac{1}{2}\beta N^{-\alpha}\right)$ for conciseness.  Recall that $\bm{S}$ follows the stationary distribution of $\left\{\bm{S}(t) \colon t \geq 0\right\}$.  To couple $\left\{\bm{S}(t) \colon t \geq 0\right\}$ with the fluid model, we solve for a function $g$ such that
\begin{equation}\label{eq:Poisson-equation}
\begin{split}
\overline{G}g(x)&=\max\left\{x-\eta, 0\right\},\\
g(0)&=0.
\end{split}
\end{equation}
It is not hard to see that the solution is
\begin{equation}
g(x) = \frac{(x - \eta)^2}{2(-\delta)}\mathds{1}_{\left\{x \geq \eta\right\}}.
\end{equation}
\end{sloppypar}

\begin{sloppypar}
Now we utilize this function $g$ to bound $\expect\left[\max\left\{\sum_{i=1}^b S_i -\eta, 0\right\}\right]$ through generator approximation.  Let $G$ be the generator of $\left\{\bm{S}(t)\colon t\ge 0\right\}$.  Then
\begin{equation*}
Gg\left(\sum_{i=1}^b s_i\right) = \sum_{\bm{s}' \in \mathcal{S}} r_{\bm{s} \to \bm{s}'}\left(g\left(\sum_{i=1}^b s'_i\right) - g\left(\sum_{i=1}^b s_i\right)\right),
\end{equation*}
where $r_{\bm{s} \to \bm{s}'}$ is the transition rate from state $\bm{s}$ to $\bm{s}'$. Since $g\left(\sum_{i=1}^b s_i\right)$ is bounded on $\mathcal{S}$, it holds that 
\begin{equation}
\mathbb{E}\left[Gg\left(\sum_{i=1}^b S_i\right)\right] = 0.
\end{equation}
Combining this with the equations in \eqref{eq:Poisson-equation} gives,
\begin{align}
\mathbb{E}\left[\max\left\{\sum_{i=1}^b S_i - \eta,0\right\}\right]
&= \mathbb{E}\left[\overline{G}g\left(\sum_{i=1}^b S_i\right)\right]\nonumber\\
&= \mathbb{E}\left[\overline{G}g\left(\sum_{i=1}^b S_i\right)- Gg\left(\sum_{i=1}^b S_i\right)\right]\nonumber\\
&= \mathbb{E}\left[g'\left(\sum_{i=1}^b S_i\right)(-\delta) - Gg\left(\sum_{i=1}^b S_i\right)\right].\label{eq:generator-approx}
\end{align}
This is what is referred to as a \emph{generator approximation} since we are approximating the generator $G$ with $\overline{G}$.
\end{sloppypar}


Next we take a closer look at the term $Gg\left(\sum_{i=1}^b S_i\right)$ and derive an upper bound for \eqref{eq:generator-approx}.
Let $P_A(\bm{s})$ be the probability that a job arrival is admitted into the system given that the system is at state $s$, i.e., the probability that all the tasks of the job are routed to positions below $b$.  Then
\begin{align*}
Gg\left(\sum_{i=1}^b s_i\right) &= \frac{N\lambda}{k} P_A(\bm{s})\left(g\left(\sum_{i=1}^b s_i + \frac{k}{N}\right) - g\left(\sum_{i=1}^b s_i\right)\right)+ Ns_1\left(g\left(\sum_{i=1}^b s_i - \frac{1}{N}\right) - g\left(\sum_{i=1}^b s_i\right)\right),
\end{align*}
where first term is the drift due to a job arrival and the second term is due to a task departure.
To derive an upper bound on \eqref{eq:generator-approx}, we divide the discussion into the three cases below.  Recall that $g(x)=\frac{(x-\eta)^2}{2(-\delta)}\mathds{1}_{\{x\ge \eta\}}$ and $g'(x)=\frac{x-\eta}{-\delta}\mathds{1}_{\{x\ge \eta\}}$.

\noindent\textbf{Case 1}: $\sum_{i=1}^b S_i < \eta - \frac{k}{N}$. In this case, clearly $g'\left(\sum_{i=1}^b S_i\right) = 0$ and $Gg\left(\sum_{i=1}^b S_i\right) = 0$.

\noindent\textbf{Case 2}: $\sum_{i=1}^b S_i \in [\eta - \frac{k}{N}, \eta + \frac{1}{N})$. By the mean value theorem,
\begin{align}
%&\mspace{21mu
g'\left(\sum_{i=1}^b S_i\right)(-\delta) - Gg\left(\sum_{i=1}^b S_i\right)%\nonumber\\
&= g'\left(\sum_{i=1}^b S_i\right)(-\delta) - \left(\frac{N\lambda}{k}P_A(\bm{S})\frac{k}{N}g'(\xi) + NS_1\frac{-1}{N}g'(\tilde{\xi})\right)\nonumber\\
&\le g'\left(\sum_{i=1}^b S_i\right)(-\delta) - \lambda g'(\xi) + S_1g'(\tilde{\xi}),\label{eq:case-2}
\end{align}
where $\xi \in \left(\sum_{i=1}^b S_i, \sum_{i = 1}^b S_i + \frac{k}{N}\right)$, $\tilde{\xi} \in \left(\sum_{i=1}^b S_i - \frac{1}{N}, \sum_{i = 1}^b S_i\right)$, and \eqref{eq:case-2} is true since $P_A(\bm{S})\le 1$ and $g'(x)\le 0$ for all $x$.

\noindent\textbf{Case 3}: $\sum_{i=1}^b S_i \geq \eta + \frac{1}{N}$. Since $g'(x)$ is continuous for all $x$, by the second order Taylor expansion in the Lagrange form,
\begin{align}
&\mspace{23mu}g'\left(\sum_{i=1}^b S_i\right)(-\delta) - Gg\left(\sum_{i=1}^b S_i\right)\nonumber\\
&= g'\left(\sum_{i=1}^b S_i\right)(-\delta) -\frac{N\lambda}{k}P_A(\bm{S})\left( \frac{k}{N}g'\left(\sum_{i=1}^b S_i\right) + \frac{k^2}{2N^2}g''(\zeta)\right)%\nonumber\\
%&\mspace{21mu}
-NS_1\left(\frac{-1}{N}g'\left(\sum_{i=1}^b S_i\right) + \frac{1}{2N^2}g''(\tilde{\zeta})\right)\nonumber\\
&\le g'\left(\sum_{i=1}^b S_i\right)\left(-\delta - \lambda + S_1\right) - \frac{1}{2N}\left(\lambda k g''(\zeta) + S_1g''(\tilde{\zeta})\right),
\end{align}
where $\zeta \in \left(\sum_{i=1}^b S_i, \sum_{i = 1}^b S_i + \frac{k}{N}\right)$, $\tilde{\zeta} \in \left(\sum_{i=1}^b S_i - \frac{1}{N}, \sum_{i = 1}^b S_i\right)$.


Combining these three cases yields
\begin{align}
&\mspace{23mu}\mathbb{E}\left[g'\left(\sum_{i=1}^b S_i\right)(-\delta) - Gg\left(\sum_{i=1}^b S_i\right)\right]\nonumber\\
&\le\mathbb{E}\left[\left(g'\left(\sum_{i=1}^b S_i\right)(-\delta)-\lambda g'(\xi) + S_1g'(\tilde{\xi})\right)\mathds{1}_{\left\{\sum_{i=1}^b S_i \in [\eta - \frac{k}{N}, \eta + \frac{1}{N})\right\}}\right]\label{termC}\\
&\mspace{21mu}-\frac{1}{2N}\mathbb{E}\left[(\lambda k g''(\zeta) + S_1g''(\tilde{\zeta}))\mathds{1}_{\left\{\sum_{i=1}^b S_i \geq \eta + \frac{1}{N}\right\}}\right] \label{termB}\\
&\mspace{21mu}+\mathbb{E}\left[g'\left(\sum_{i=1}^b S_i\right)(-\delta - \lambda + S_1) \mathds{1}_{\left\{\sum_{i=1}^b S_i \geq \eta + \frac{1}{N}\right\}}\right].\label{termA}
\end{align}

The first two terms \eqref{termC} and \eqref{termB} are easy to bound once we notice that for any $x \in \left[\eta - \frac{k + 1}{N},\eta + \frac{k + 1}{N}\right]$, $|g'(x)| \leq \frac{|x - \eta|}{\delta} \leq \frac{1}{\sqrt{N}\log N}$, and for any $x \in (\eta, +\infty)$, $|g''(x)| = \frac{1}{\delta} = \frac{\sqrt{N}}{(k + 1)\log N}$.
Then when $N$ is sufficiently large,
\begin{align}
|\eqref{termC}| &\leq \frac{1}{\sqrt{N}\log N}\left(\frac{(k+1)\log N}{\sqrt{N}}+1+1\right)\le\frac{3}{\sqrt{N}\log N}\nonumber,
\end{align}
and
\begin{align}
|(\ref{termB})| &\leq \frac{1}{2N}\frac{\sqrt{N}}{(k+1)\log N}\left(\lambda k + 1\right) \leq \frac{1}{\sqrt{N}\log N}.\nonumber
\end{align}

The \emph{key} in this proof is to bound the term \eqref{termA}, for which we utilize the state-space collapse result we establish in Lemma~\ref{lem:ssc} below.  The proof of Lemma~\ref{lem:ssc} is given in Appendix~\ref{app:lemma:ssc}.
\begin{lemma}[State-Space Collapse]\label{lem:ssc}
Under the assumption of Theorem \ref{main_theorem_1}, consider the following Lyapunov function:
$$
V(\bm{s}) = \min\left\{\frac{1}{h - 1}\sum_{i=h}^b s_i, b\left(\left(1 - \frac{1}{2}\beta N^{-\alpha}\right) - \frac{1}{h-1}\sum_{i=1}^{h - 1} s_i\right)^+\right\},
$$
where the superscript $^+$ denotes the function $x^+=\max\{x,0\}$.
Let $B = \frac{b - h + 1}{h - 1}\left(\beta N^{-\alpha} + \frac{\log N}{\sqrt{N}}\right)$. Then for any state $\bm{s}$ such that $V(\bm{s}) > B$, its Lyapunov drift can be upper bounded as follows
$$
\Delta V(\bm{s}) = GV(\bm{s}) \leq -\frac{b}{\sqrt{N}}.
$$
Consequently, when $N$ is sufficiently large,
\begin{align*}
\Pr\left\{V(\bm{S}) > B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}\right\}\le e^{-\frac{1}{2}\log^2 N}.
\end{align*}
\end{lemma}

With Lemma~\ref{lem:ssc}, we partition the probability space based on the value of $V(S)$ for bounding \eqref{termA}.  Note that $g'\left(\sum_{i=1}^b S_i\right)(-\delta - \lambda + S_1) \mathds{1}_{\left\{\sum_{i=1}^b S_i \geq \eta + \frac{1}{N}\right\}}$ is always no larger than $\frac{2b}{\delta}$ for large enough $N$.  Then \eqref{termA} can be upper bounded as:
\begin{align}
\eqref{termA}&\le \mathbb{E}\left[g'\left(\sum_{i=1}^b S_i\right)(-\delta - \lambda + S_1)%\right.\nonumber\\
%&\mspace{42mu}\left.
\cdot\mathds{1}_{\left\{\sum_{i=1}^b S_i \geq \eta + \frac{1}{N}\right\}}\;\middle|\; V(\bm{S}) \le B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}\right]\nonumber\\
&\mspace{21mu}+\frac{2b}{\delta}\Pr\left\{V(\bm{S}) > B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}\right\}.\label{eq:upper-termA}
\end{align}
Now we focus on the case where we are given the condition that $V(\bm{S}) \le B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}$.  Our goal is to show that $S_1$ is large enough such that $\delta+\lambda-S_1<0$.  Intuitively, this condition on $V(\bm{S})$ implies that we either have a small $\sum_{i=h}^b S_i$, which leads to a large $S_1$ when combined with the condition $\sum_{i=1}^b S_i \geq \eta + \frac{1}{N}$ in the indicator, or a large $\sum_{i=1}^{h - 1} S_i$, which directly gives a large $S_1$ since $S_1\geq \cdots\ge S_{h - 1}$.

\begin{sloppypar}
If $\frac{1}{h - 1}\sum_{i=h}^b S_i \le  b\left(\left(1 - \frac{1}{2}\beta N^{-\alpha}\right) - \frac{1}{h-1}\sum_{i=1}^{h - 1} S_i\right)^+$ in $V(\bm{S})$, the condition $V(\bm{S}) \le B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}$ implies that
\begin{equation}\label{eq:left-small}
\frac{1}{h - 1}\sum_{i=h}^{b} S_i \leq \frac{b - h + 1}{h - 1}\left(\beta N^{-\alpha} + \frac{\log N}{\sqrt{N}}\right) + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}.
\end{equation}
Recall that $b = \min\left\{N^{\alpha},\frac{N^{0.5-\alpha}}{k}\right\}$ and $h = o(\log k)$.  Note that the indicator function in \eqref{eq:upper-termA} makes it sufficient to consider the case where $\sum_{i=1}^b S_i \geq \eta + \frac{1}{N}$, which implies $(h-1)S_1+\sum_{i=h}^b S_i \geq \eta$.  Combining this with \eqref{eq:left-small} gives
\begin{align*}
S_1&\ge\frac{\eta}{h-1}-\frac{b - h + 1}{h - 1}\left(\beta N^{-\alpha} + \frac{\log N}{\sqrt{N}}\right) - \frac{2kb\log^2 N}{(h-1)\sqrt{N}}\\
&\ge 1 + (1-\beta)\frac{1}{h-1}-\frac{1}{2}\beta N^{-\alpha} + o\left(\frac{1}{h}\right)
\end{align*}
when $N$ is sufficiently large.  Note that $\delta=o\left(\frac{1}{h}\right)$ and $\lambda=1-\beta N^{-\alpha}$.  Therefore, $\lambda + \delta - S_1 < 0$ when $N$ is sufficiently large.
\end{sloppypar}


\begin{sloppypar}
If $\frac{1}{h - 1}\sum_{i=h}^b S_i >  b\left(\left(1 - \frac{1}{2}\beta N^{-\alpha}\right) - \frac{1}{h-1}\sum_{i=1}^{h - 1} S_i\right)^+$ in $V(\bm{S})$, the condition $V(\bm{S}) \le B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}$ implies that
\begin{align*}
b&\left(1 - \frac{1}{2}\beta N^{-\alpha}-\frac{1}{h-1}\sum_{i=1}^{h-1} S_i\right) \le B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}.
\end{align*}
Then
\begin{align*}
S_1 &\ge \frac{1}{h-1}\sum_{i=1}^{h-1} S_i\\
&\ge 1 - \frac{1}{2}\beta N^{-\alpha} - \frac{1}{b}\left(B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}\right) \\
&\geq 1 - \frac{1}{2}\beta N^{-\alpha} + o(N^{-\alpha}).
\end{align*}
As a result, again we have $\lambda + \delta - S_1 \leq -\frac{1}{2}\beta N^{-\alpha} + o(N^{-\alpha}) < 0$ when $N$ is sufficiently large.
\end{sloppypar}

Inserting these bounds back to \eqref{eq:upper-termA} gives that when $N$ is sufficiently large,
\begin{align*}
\eqref{termA} &\le 0 + \frac{2b}{\delta}\Pr\left\{V(\bm{S}) > B + \frac{2kb\log^2 N}{(h-1)\sqrt{N}}\right\}\\
&\le \frac{2b}{\delta}e^{-\frac{1}{2}\log^2 N}\\
&\leq \frac{1}{\sqrt{N}\log N}.
\end{align*}


Combining the bounds for \eqref{termC}, \eqref{termB} and \eqref{termA}, we have
$$
\mathbb{E}\left[\max\left\{\sum_{i=1}^b S_i - h\left(1-\frac{1}{2}\beta N^{-\alpha}\right), 0\right\}\right] \le \frac{5}{\sqrt{N}\log N},
$$
which completes the proof of Theorem \ref{main_theorem_1}.
\end{proof}

==> Achieving Zero Queueing Delay for Parallel Jobs/proof-theorem_zero_delay.tex <==
\begin{proof}
We first bound the dropping probability $\probdrop$ using Lemma~\ref{lem:filling} with the threshold value $\ell=b$.  Note that an incoming job does not get dropped if and only if all its $k$ tasks are routed to queueing positions below threshold $b$, which is the complement of the event $\textrm{FILL}_b$ in Lemma~\ref{lem:filling}. Thus,
\begin{align*}
\probdrop&=1-\Pr\{\textrm{FILL}_b\}\\
&=1-\Pr\left\{\textrm{FILL}_b\;\middle|\; \sum_{i=1}^b S_i \le b\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}%\\
%&\mspace{48mu}
\cdot\Pr\left\{\sum_{i=1}^b S_i \le b\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}\\
&\mspace{23mu}-\Pr\left\{\textrm{FILL}_b\;\middle|\; \sum_{i=1}^b S_i > b\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}%\\
%&\mspace{36mu}
\cdot\Pr\left\{\sum_{i=1}^b S_i > b\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}.
\end{align*}
We can easily have that $\Pr\left\{\textrm{FILL}_b\;\middle|\; \sum_{i=1}^b S_i \le b\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}\le \frac{1}{N}$ using Lemma~\ref{lem:filling}.

Now we bound $\Pr\left\{\sum_{i=1}^b S_i > b\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}$ using Theorem~\ref{main_theorem_1}.  Note that
\begin{align*}
&\mspace{23mu}\Pr\left\{\sum_{i=1}^b S_i > b\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}\\
&\le \Pr\left\{\max\left\{\sum_{i=1}^b S_i - h\left(1 - \frac{1}{2}\beta N^{-\alpha}\right),0\right\}> b - \frac{b}{4}\beta N^{-\alpha}-h\right\}\\
&\le \Pr\left\{\max\left\{\sum_{i=1}^b S_i - h\left(1 - \frac{1}{2}\beta N^{-\alpha}\right),0\right\}> \frac{b}{2}\right\},
\end{align*}
where we have used the fact that $\frac{b}{4}\beta N^{-\alpha}+h\le \frac{b}{2}$ when $N$ is sufficiently large due to our assumptions on $b$ and $h$.  Then by Markov's inequality,
\begin{align*}
%&\mspace{23mu}
\Pr\left\{\sum_{i=1}^b S_i > b\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}%\\
&\le\frac{\expect\left[\max\left\{\sum_{i=1}^b S_i - h\left(1 - \frac{1}{2}\beta N^{-\alpha}\right),0\right\}\right]}{\frac{b}{2}}\\
&\le \frac{10}{b\sqrt{N}\log N}.
\end{align*}

Combining the arguments above yields
\begin{align*}
\probdrop\ge 1-\frac{1}{N}-\frac{10}{b\sqrt{N}\log N}\ge 1-\frac{11}{b\sqrt{N}\log N}
\end{align*}
when $N$ is sufficiently large.

Next we bound the expected job delay given that a job is admitted, i.e., $\expect[T\;|\;\textup{admitted}]$.  We define the delay of a job that is dropped to be zero since it leaves the system immediately after arrival.  Then $\expect[T]=\expect[T\;|\;\textup{admitted}]\cdot(1-\probdrop)+\expect[T\;|\;\textrm{dropped}]\cdot\probdrop$, and thus $\expect[T\;|\;\textup{admitted}]=\frac{\expect[T]}{1-\probdrop}$.  So we can focus on bounding $\expect[T]$, following the outline given in the proof sketch.

We bound $\expect[T]$ in the following way
\begin{align}
\mathbb{E}[T] &\leq \mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right]\label{eq:term-fill}\\ 
&\mspace{21mu}+ \mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i > h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right]%\nonumber\\
%&\mspace{36mu}
\cdot\Pr\left\{\sum_{i=1}^h S_i > h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}.\label{eq:term-not-fill}
\end{align}

For the first term \eqref{eq:term-fill} in this upper bound, as described in the proof sketch, we will rely on the fact that with high probability, all the $k$ tasks are assigned to queueing positions below $h$.  Specifically,
\begin{align*}
&\mspace{22mu}\mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right]\\
&=\mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right),\textrm{FILL}_h\right]%\\
%&\mspace{23mu}
\cdot\Pr\left\{\textrm{FILL}_h\;\middle|\;\sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}\\
&\mspace{23mu}+\mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right),\overline{\textrm{FILL}_h}\right]%\\
%&\mspace{46mu}
\cdot\Pr\left\{\overline{\textrm{FILL}_h}\;\middle|\;\sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\},
\end{align*}
where $\overline{\textrm{FILL}_h}$ is the complement of $\textrm{FILL}_h$.

Suppose $\textrm{FILL}_h$ is true.  Suppose that the $k$ tasks of the incoming job land in $m$ distinct queues with $m\le k$.  We call the tasks with the highest positions in these $m$ queues tasks $1,2,\dots,m$, and let $n_1,n_2,\dots,n_m$ denote these positions.  Then the delay of task $i$ can be written as $Y_i=\sum_{j=1}^{n_i}X_{i,j}$, where $X_{i,j}$ is the service time of the task at position $j$ in the same queue as task $i$.  Clearly $X_{i,j}$'s are i.i.d.\ with an exponential distribution of rate $1$.  We know that $n_i\le h, i=1,2,\dots,m$ given $\textrm{FILL}_h$.  Then by Lemma~\ref{lem:max-upper},
$$
\mathbb{E}[\max\left\{Y_1,\cdots,Y_m\right\}] \leq \ln k + o(\ln k).
$$

\begin{sloppypar}
When $\overline{\textrm{FILL}_h}$ is true, $\mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right),\overline{\textrm{FILL}_h}\right]\le bk$ since the highest position for a task is $b$ and the maximum is upper bounded by the sum.  Further, $\Pr\left\{\overline{\textrm{FILL}_h}\;\middle|\;\sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}\le \frac{1}{N}$ by Lemma~\ref{lem:filling}.
\end{sloppypar}

Combining the arguments above, we have the following bound for term \eqref{eq:term-fill}:
\begin{align*}
\mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i \leq h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right]\le \ln k+o(\ln k)+\frac{bk}{N}.
\end{align*}


Now we go back to the term \eqref{eq:term-not-fill}.  Again, it is easy to see that $\mathbb{E}\left[T \;\middle|\; \sum_{i=1}^h S_i > h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right]\le bk$.  Utilizing Theorem~\ref{main_theorem_1}, we have
\begin{align*}
%&\mspace{23mu}
\Pr\left\{\sum_{i=1}^h S_i > h\left(1 - \frac{1}{4}\beta N^{-\alpha}\right)\right\}%\\
&\le \Pr\left\{\max\left\{\sum_{i=1}^b S_i-h\left(1-\frac{1}{2}\beta N^{-\alpha}\right),0\right\} > \frac{1}{4}h\beta N^{-\alpha}\right\}\\
&\le\frac{\expect\left[\max\left\{\sum_{i=1}^b S_i-h\left(1-\frac{1}{2}\beta N^{-\alpha}\right),0\right\}\right]}{\frac{1}{4}h\beta N^{-\alpha}}\\
&\le \frac{20}{h\beta N^{\frac{1}{2}-\alpha}\log N}.
\end{align*}

With the bounds above on \eqref{eq:term-fill} and \eqref{eq:term-not-fill}, we have
\begin{equation*}
\expect[T]\le \ln k+o(\ln k)+\frac{bk}{N}+\frac{20bk}{h\beta N^{\frac{1}{2}-\alpha}\log N}.
\end{equation*}
Consequently,
\begin{align*}
\expect[T\;|\; \text{admitted}]&=\frac{\expect[T]}{1-\probdrop}\\
&\le \frac{\ln k+o(\ln k)+\frac{bk}{N}+\frac{20bk}{h\beta N^{\frac{1}{2}-\alpha}\log N}}{{1-\probdrop}}\\
&\le \ln k + o(\ln k),
\end{align*}
which completes the proof.
\end{proof}

==> Achieving Zero Queueing Delay for Parallel Jobs/response-letter.tex <==

{\color{blue}
We would like to thank the reviewers and the TPC chairs for the constructive comments and suggestions.  We have carefully revised our paper to address the one-shot revision requirements and the individual comments from the reviewers.  Some key highlights of the changes are summarized below:
\begin{itemize}[leftmargin=1em]
    \item We have conducted simulation experiments based on the suggestions of the reviewers and added Section~7 to present the results.  Through the simulations, we are able to demonstrate the consistency between numerical results and our theoretical results under reasonable settings, and to address some gaps in the theoretical analysis.
    \item We have added Section~6 to discuss the more stringent notion of zero queueing delay mentioned by the reviewers that requires all the tasks of a job to have zero waiting time in queues.
    \item We have made major adjustments to the structure of the paper to make the proofs of the main results more accessible.  These adjustments include developing more understanding of zero queueing delay on a job level at the beginning of Section~4, sketching the proofs before presenting the formal proofs in Sections~4 and 5, and moving lemmas and their proofs to the appendix.
    \item We have added many intuitions, explanations, clarifications, and justifications throughout the paper.
\end{itemize}

Below we first give our detailed responses to the one-shot revision requirements.  Then we will address the individual comments of each of the reviewers, focusing more on the comments that are not addressed in our responses to the one-shot revision requirements.  Our responses are in blue and the quoted requirements/comments are in black.  We also highlighted major changes in the paper in blue text.}


\section*{One-Shot Revision Requirements}

The one-shot revision requires the authors to address all the comments in each of the reviews and to add a detailed set of numerical experiments that address the important points below. Acceptance is contingent on the authors making these required changes.

In addressing all the reviewer comments, the authors must specifically address the following points:
{\color{blue} (We have added a prefix ``I.'' to the indices of the comments for ease of reference.)}
\begin{enumerate}[label=\textbf{(I.\alph*)},leftmargin=2.1em]
    \item The presentation and structure of the paper needs to be improved. Some or all of the proofs should be deferred to an appendix, and instead in the main body of the paper the authors could provide a sketch of the proof (or a high-level explanation) and provide more insights on the performance. The extra space should be devoted for a numerical section.
    
    {\color{blue} We have made the following major adjustments to the structure of the paper to improve the presentation based on the comments and suggestions of the reviewers:
    \begin{itemize}[leftmargin=1em]
        \item For proving the achievability results, we have added three segments at the beginning of Section~4 (Pages 8--10) to develop more understanding on how zero queueing delay relates to the system state, and to provide a proof sketch.  We have then moved an additional lemma and the proofs of all the lemmas involved to Appendix~A.  However, the proofs of Theorems~3.1 and 3.2 remain in this section since we deem them as essential for understanding the theoretical results of the paper, which constitute a main part of the contributions of the paper.
        
        \item For proving the impossibility results, we have added a proof sketch at the beginning of Section~5 (Page~16) to help guide the readers through the proofs.  Again, we have moved the lemmas and their proofs to Appendix~B, but have kept the proofs of Theorems~3.3 and 3.4.  The proof techniques for Theorem~3.3 are novel and we believe that they could be of interest to many readers.
        
        \item As we summarized at the beginning of this response letter, we have added simulation results (Section~7) and discussion on another notion of zero queueing delay (Section~6), and have made an effort to provide insights by integrating many intuitions, explanations, clarifications, and justifications throughout the paper.  More details can be found in our responses to other revision requirements.
    \end{itemize}
    }
    
    \item The notation used in the paper should be defined.
    
    {\color{blue} We have added a paragraph as a reminder to Bachmann--Landau asymptotic notation in Section~1 right before the related work subsection (Page~4).  We have also added clarifications on the definition of the generator of the fluid model in Section~4.1 (Page~10).  %%Other notation missing?
    }
    
    \item The paper claims that their modeling assumptions are more realistic than those previously considered in the literature. This claim needs to be better substantiated. The authors should carefully justify their model providing examples in which the model can be applied. 
    
    {\color{blue}
    We address this comment for the following modeling assumptions.
    \begin{itemize}[leftmargin=1em]
        \item The main modeling assumption that differentiates our paper from papers in the literature is the parallel job assumption, i.e., we assume that each job can be parallelized into multiple tasks.  This assumption reflects the widely adopted parallel computing framework in many applications.  We have added more references in Section~1 (Page~2) to justify the predominance of such a model and to give application examples (distributed cloud computing, distributed file systems, machine learning systems).
        
        For such a model with parallel jobs, we need to choose the performance metric properly.  In this paper, we focus on the delay of jobs rather than the delay of tasks since usually a job is a meaningful unit for users.  Our choice is in line with the design goal of many practical schedulers (examples given in Section~1 on Page~2).
        
        However, despite the popularity of parallelism in practice, there is a significant gap in the literature of queueing theory/stochastic systems, where jobs that can be parallelized have not been extensively studied.  There is very limited amount of prior work that considers parallel jobs and analyzes job delay, and the very few papers that do analyze job delay have only got fluid-level optimality at the best and have only considered a constant load.
        We have added a bit more emphasis on this when discussing the challenges and our results in Section~1 (before the reminder of Bachmann-Landau notation on Page~4).
        
        \item Another modeling assumption we make is that the task service times are i.i.d.\ exponential.  We would like to clarify that we did not claim that this modeling assumption is more realistic than those previously considered, since it is a rather typical assumption made in theoretical studies.  However, we are able to use simulations to empirically
        investigate how the service time distribution affects the trend of queueing delay.  We have added simulations in Section~7.2 to experiment on hyper-exponential distributions and bounded Pareto distributions as distributions for task service times.  The simulation results show that the queueing delay also has a trend to converge to zero under these two distributions.  We leave the theoretical analysis under these distributions and also correlated service times as future research directions.
        
        \item We assume that $k$, the number of tasks in a job, scales with $N$, the number of servers.  The motivation for this modeling assumption is to capture the increasing size of jobs as the computing power grows.  We have added some clarifications throughout the paper to make this assumption even more explicit.  Since studies on parallel jobs are scarce, it is hard to conclude if this assumption is more realistic than those in existing work or not.  In fact, we hope that our paper can serve as a first step towards characterizing behaviors under different scaling regimes.
        
    \end{itemize}
    }
    
    \item The paper considers a specific form of zero queueing delay that actually allows tasks in a job to wait in queues for non-negligible amounts of time. The paper should mention other possible forms of zero queueing delay that are more stringent, and discuss how the analysis presented in the paper might be extended to address these more stringent forms of zero queueing delay.
    
    {\color{blue}
    We have added a section (Section~6, Page~19) to discuss the more stringent notion where all the tasks of a job need to be assigned to idle servers.  We show an impossibility result that this more stringent notion cannot be achieved when the probe overhead is $O(\frac{1}{1-\lambda})$.  However, we wanted to point out that although this notion seems to be similar to the notion of zero queueing for non-parallel (single-task) jobs, the two systems have fundamentally different dynamics and thus it is hard to make an analogy.  We would like to also argue that the notion we proposed that compares the actual job delay with the hypothetical job delay assuming no queueing is more natural and thus remains the focus of the paper.  As we explained in the first bullet point above, performance on a job level is what the users care the most, and this is reflected in the design goal of many practical schedulers.  We also address the comparison with single-task setting in the comment (I.e) below. 
    }
    
    \item  One of the main claims of the paper is that thanks to parallelization, asymptotic zero queueing delay is obtained with lower overhead than in the single-task setting. However, the performance metric is looser than in the related literature, where typically the waiting time is shown to be $0$ asymptotically, and hence the comparison is not fair. This needs to be clearly explained throughout the paper. In addition, the revision should address this issue and provide evidence that parallelization will also achieve $0$ waiting time asymptotically (all tasks should find an empty server, except those that are not the head-of-the-line in the batch). In order to achieve this, the revision should carry out the analysis of the parallelization scheme for the waiting time.
    
    {\color{blue}
    First, we would like to clarify that it is hard to conclude that our notion of zero queueing delay is looser than in the related literature since the majority of existing work considers non-parallel (single-task) jobs.  We have added explanations on how a system with parallel jobs has fundamentally different dynamics from a system with non-parallel jobs (paragraphs under ``Challenges and our results'' in Section~1 on Page~3, Section~6).  We have also added clarifications on how our notion is different from the conventional notion for non parallel jobs (blue paragraph at the top of Page~3).
    
    We respectfully disagree that parallelization needs to necessarily guarantee that all tasks find empty servers.  As we argued in the response to comment (I.c) above, it is much more typical that users consider performance on a job level.
    
    We wanted to add that we may be able to address this comment better if the reviewers can clarify what they refer to as tasks ``that are not the head-of-the-line in the batch.''  Tasks of the same job arrive together and there is no particular ordering among them.
    }
\end{enumerate}

The authors must conduct numerical experiments whose results confirm and demonstrate all the claims of the paper based on the asymptotic results for realistic parameter values. Of particular importance for parameter values is the number of parallel tasks $k$ and showing that all the claims of the paper hold for moderately large values of $k$. In addition, the authors must conduct corresponding numerical experiments for increasingly larger values of $k$ and $N$ to demonstrate how these numerical results approach the asymptotic results and to provide an understanding of the convergence behavior toward the asymptotic results. In conducting these numerical experiments, it is of particular interest for the authors to address the following points:
{\color{blue} (We have added a prefix ``II.'' to the indices of the comments for ease of reference.)}
\begin{enumerate}[label=\textbf{(II.\alph*)},leftmargin=2.6em]
\item One of the main claims of the paper is that thanks to parallelization, asymptotic zero queueing delay is obtained with lower overhead than in the single-task setting. However, the performance metric is looser than in the related literature, where typically the waiting time is shown to be $0$ asymptotically, and hence the comparison is not fair. If it is not possible to carry out the analysis of the parallelization scheme to achieve $0$ waiting time asymptotically (all tasks should find an empty server, except those that are not the head-of-the-line in the batch) as noted above, then the paper should explain the reasons for this and the numerical experiments should assess whether parallelization also achieves asymptotically $0$ waiting delay, and if it does, further assess the overhead required for it.

{\color{blue}Please refer to our responses to comments (I.d) and (I.e) in the last group of comments.  Since we feel that we have addressed this concern sufficiently, we did not perform further numerical experiments.
}

\item There seems to be a gap between the regimes in which the asymptotic relative delay vanishes, and when it doesn't. As parameters such as $k$ and $N$ are increased, the numerical experiments should investigate this gap. As parameters such as $k$ and $N$ are increased, the numerical experiments should investigate the gap in the bounds and provide an understanding of the convergence behavior toward the asymptotic results.

{\color{blue}
We thank the reviewers for this great suggestion.  We have added simulation experiments for different scalings of the probe ratio $d$ to investigate this gap.  Please see Section~7.1 on Pages~19--20 for the details.  A quick summary is that for a probe ratio that satisfies the conditions for achievability (Theorems~3.1 and 3.2), the empirically trend of queueing delay is consistent with the theoretical results; the simulation results suggest that our impossibility results are not tight, which causes the gap.  These simulation results serve as great guidelines for future research directions.
}

\item With the unfair queueing delay comparison, the total service requirement of a job being smaller than its original size and other differences between the single-task and parallel-tasks setting (see reviewer comments), it is important to pinpoint the main reasons for the differences in the asymptotic behavior. The numerical experiments should investigate and identify the main reasons for these differences.

{\color{blue}
For whether our notion of zero queueing delay induces fair comparisons, please refer to our responses to comments (I.d) and (I.e) in the last group of comments.

We would like to make some clarifications regarding the concern related to the total service requirement.  When a job is parallelized, its total size is not altered, but the job can be served by multiple servers simultaneously in parallel.  We agree that when there is no queueing, the job delay after parallelization becomes smaller than that in the case of no parallelization, which is the motivation for parallelization.  Our notion of zero queueing delay is relative to the job delay under parallelization, which should not cause unfairness towards our favor in our opinion.

We would like to argue that this reduction in probe overhead reflects the overall effect of parallelization on the system.
There are several factors at play that are brought by parallelization all together.  This makes it hard to quantify their individual effects through numerical experiments since it is hard if not impossible to take away one factor without affecting other factors.

We list those factors below.  First, for tasks of the same job, the probe overhead quota is pooled together and their assignment is coordinated, leading to a more effective use of the state information.  Second, a job with parallel tasks can better tolerate task delays since the job delay is anyway determined by the slowest task.  Furthermore, work arrives to the system in a more bursty fashion under parallelization due to the batch effect.

We have added this discussion in the ``Challenges and our results'' subsection of Section~1 on Pages~3--4.
}


\item Include a discussion of the comparison between the numerical results and theoretical results and an understanding that is provided by this comparison.

{\color{blue} We have included such discussions throughout the added section for simulation results (Section~7).
}

\end{enumerate}


It is important to emphasize that acceptance is contingent on the numerical experiments confirming and demonstrating all the claims of the paper based on the asymptotic results for realistic parameter values and demonstrating how these numerical results approach the asymptotic results for increasingly larger values of these parameter values.

{\color{blue} We thank the reviewers again for the suggestions on numerical experiments.  We found the comparisons of theoretical results and simulation results very inspiring.  We hope that the readers will be able to gain more understanding and insights from this added section.
}


\section*{Reviewers' Comments}

\subsection*{Review \#67A}
\textbf{Paper summary}

This paper studies a queueing system with $N$ servers in which upon arrival of a job, $d$ servers are probed, and $k <d$ tasks of the job are dispatched to the servers with shortest queue-lengths. A job is completed when all of its $k$ tasks finish service. In an asymptotic regime in which $k$, $d$, and $N$ tend to infinity, the paper shows that under suitable choice of $d$ and $k$, the relative difference between the obtained delay and the minimum achievable one tends to $0$. 

The theoretical contribution is sound, but not a breakthrough in the light of recent papers that have obtained results of similar nature. The paper lacks a numerical section, and in my view, the theoretical contribution in itself is not significant enough to warrant publication in Sigmetrics.

{\color{blue} \noindent\textbf{Response.}
We have added explanations on how a system with parallel jobs has fundamentally different dynamics from a system with non-parallel jobs and why that makes the analysis more challenging.  Please refer to the ``Challenges and our results'' subsection of Section~1 on Pages~3--4 for more details.  We have added a numerical section as Section~7.  Please refer to the responses to the one-shot revision requirements and Section~7 on Pages~19--20 of the paper for more details.
}

\noindent\textbf{What are the strengths of the paper?}

Sound theoretical analysis of a model of practical interest.

\noindent\textbf{What area of the paper need improvement?}

A numerical section would have been appreciated provide more insights into the performance of the system. See details below.

{\color{blue} \noindent\textbf{Response.}  Please refer to our responses to the one-shot revision requirements for discussions on the numerical section.}

The presentation could be improved. For example, asymptotic notation is extensively used, little-o, big-O, $\omega$, $\Omega$, without ever being defined. The fact that $k$ and $d$ scale with $N$ should also made clear from the abstract on.

{\color{blue} \noindent\textbf{Response.}  We have added a paragraph as a reminder to Bachmann--Landau asymptotic notation in Section~1 right before the related work subsection (Page~4).  We have also made the fact that $k$ and $d$ scale with $N$ more explicit in the abstract and throughout the paper.
}

One of the main messages of the paper is that by parallelizing, zero queueing delay can be obtained with less overhead than in the single-task setting. However, the modeling assumptions are typically different, and as a consequence, it is not obvious to conclude that parallelizing improves the asymptotic performance. This should be explained clearly throughout.

{\color{blue} \noindent\textbf{Response.} 
Please refer to our responses to the one-shot revision requirements (I.d), (I.e) and (II.c).}



\noindent\textbf{Other comments for author}

There seems to be a gap between the regimes in which the asymptotic relative delay vanishes, and when it doesn't. This gap could have been explored numerically.

{\color{blue} \noindent\textbf{Response.}  We thank the reviewer for this great suggestion!  We have added Section~7.1 on Pages~19--20 to investigate this gap.  Please refer to our response to the one-shot revision requirement (II.b).}

The model assumes iid service times (exponential distribution) for the tasks. If the original service time of a job is 1, then the maximum of $k$ independent tasks with each a mean service requirement of $1/k$ is smaller than 1, i.e., the mean service requirement with multiple tasks is smaller than the original one. This assumption plays a key role in the analysis, and its impact could have been explored numerically, for example assuming non-exponential service times, identical copies across tasks, other correlation structure among the service times of tasks etc.

{\color{blue} \noindent\textbf{Response.}  We have added Section~7.2 (Page~20) to explore non-exponential service times.  Please also refer to the second bullet point in our response to the one-shot revision requirement (I.c).

We would like to clarify that we normalize the mean task size to be $1$.  The parallelization does affect the job delay even under no queueing.  But we believe that it does not cause unfairness towards our favor since our notion of zero queueing delay is relative to the job delay under parallelization.  Please also refer to our response to the one-shot revision requirement (II.c).
}

In papers considering the single-task case the main criteria is that the waiting probability tends to $0$, whereas in the present paper the relative delay is considered. In addition, the total service requirement of a job is smaller than its original size. It is therefore not clear to pinpoint the main reason for the difference for the difference in the asymptotic behavior. The comparison with related literature is not carried out on the same ground. This is also that could  have been further explored numerically.

{\color{blue} \noindent\textbf{Response.}  Please refer to our responses to the one-shot revision requirement (I.d), (I.e) and (II.c) for the discussions on the comparison with non-parallel models.}

The paper claims that the modeling assumptions considered (multiple tasks, iid distributed, with $d$ and $k$ scaling with $N$) are more realistic than the ones considered in previous literature. A reference is needed to support this claim, otherwise the claim should be downplayed.

{\color{blue} \noindent\textbf{Response.}  Please refer to our response to the one-shot revision requirement (I.c) for justifications of some of our modeling assumptions.
}

From Section 4.1 on, what is the generator of a fluid model? 

{\color{blue} \noindent\textbf{Response.}   We have added clarifications on the definition of the generator of the fluid model in Section~4.1 (Page~10).}

\noindent Other comments:

- Section 2, 8th line, ``when all of ITS tasks finish...''

{\color{blue} \noindent\textbf{Response.}  Fixed. Please see Page~5.}

- After eq (5). "Therefore, the batch-filling policy achieves 0 queueing delay". Is this concluded from THM 3.2, or THM 3.1? Be more specific.

{\color{blue} \noindent\textbf{Response.}  It is from Theorem~3.2.  We have made it more specific on Page~7.}




\subsection*{Review \#67B}
\noindent\textbf{Paper summary}

This paper considers a classical load balance architecture with one dispatcher and $N$ parallel homogeneous servers. Jobs arrive at the system according to a Poisson process.  Differently from the classical case jobs are not atomic objects. They can be break in $k$ tasks, which can be executed in parallel (of course, a job finishes upon the completion of the  last task). 

Authors propose  batch-filling policy, a variant of the classical Po-d (Power of d) policy, and show that  it achieves asymptotically zero queuing delay (i.e. the sojourn time of a job in the system is asymptotically dominated by its service time) as long as d is consistently chosen.


\noindent\textbf{What are the strengths of the paper?}

The paper  seems technically sound (even if I could not check completely).  Form a technical point of view results are non trivial. Even is the topic is well established, it is still a relevant topic, and any results that advances  this field can be of interest.


\noindent\textbf{What area of the paper need improvement?}

The assumption that jobs breaks into tasks that can be executed in parallel should be better motivated. For example this is true in Hadoop if reduce tasks are ignored, but can we  really ignore them?

{\color{blue}\noindent\textbf{Response.}
We thank the reviewer for this great suggestion!
We have added more references in Section~1 (Page~2) to justify the predominance of such a model and to give application examples (distributed cloud computing, distributed file systems, machine learning systems).

We agree that the reduce tasks cannot be really ignored in Hadoop.  However, we would like to think that our analysis can be applied to study the completion time of the map phase, which can provide a good basis for further analysis on the overall delay.  More generally, we hope that our analysis can contribute towards understanding parallel jobs with more complicated structures such as multiple stages or more general precedence relationship among tasks.
}

\noindent\textbf{Other comments for author}

I think the authors should carefully justify their model providing examples in which  their model can be applied. For the rest the paper is pretty well written (even if it is not an easy read). I have appreciated the attempt made by the authors to provide a high-level overview of the proofs  (at least for what concerns the upper-bound) before  digging deeply into details.

{\color{blue}\noindent\textbf{Response.} We thank the reviewer for appreciating our attempt to make the proofs more accessible.  We have made further changes towards this goal.  Please refer to our response to the one-shot revision requirement (I.a).
}






\subsection*{Review \#67C}
\noindent\textbf{Paper summary}

This paper revisits the well-studied problem of achieving zero asymptotic queueing delay using the power-of-d choices policy by replacing single indivisible jobs with jobs consisting of parallel tasks. The paper shows that a previously proposed variant of the power-of-d-choices policy in the literature achieves zero asymptotic queueing delay with a probe overhead for d that is an improvement over previous studies and includes the number of tasks in each job.


\noindent\textbf{What are the strengths of the paper?}

The paper revisits an important load balancing problem with the extension to parallel jobs. Theoretical results are established that support zero queueing delays for larger values of probe overhead d.

\noindent\textbf{What area of the paper need improvement?}

The paper assumes that the number of tasks per job is a fixed parameter k, not allowing the number of tasks per job to vary from parallel job to parallel job. The paper considers a specific form of zero queueing delay which allows tasks in a job to wait in queues for non-negligible amounts of time. The paper assumes Poisson arrives and exponential service, with the hope to extend the results to general service time distributions.


\noindent\textbf{Other comments for author}

The paper assumes that the number of tasks per job is a fixed parameter k. It would be interesting to extend the analysis to consider the number of tasks per job k to be sampled from a probability distribution with a given mean $\bar{k}$, and attempt to show that the established results in terms of k then hold in an appropriate sense with respect to the mean number of jobs $\bar{k}$.

{\color{blue}\noindent\textbf{Response.}
This is a very interesting proposal.  We believe that if $k$ follows a distribution with a finite support set $\{k_{\ell},k_{\ell}+1,\cdots,k_r\}$ such that $k_r \leq k_{\ell}^c$ where $c$ is a positive constant, the achievability results should still hold.  But this is a question that needs much more scrutiny and we will pursue it in future work.
}



The paper considers a specific form of zero queueing delay that actually allows tasks in a job to wait in queues for non-negligible amounts of time. The paper should mention other possible forms of zero queueing delay that are more stringent, and discuss how the analysis presented in the paper might be extended to address these more stringent forms of zero queueing delay.

{\color{blue}\noindent\textbf{Response.}
We thank the reviewer for this great suggestion!  We have added Section~6 to discuss the more stringent notion.  Please refer to our responses to one-shot revision requirements (I.d) and (I.e).
}

In section 2, there is no need to repeat the expression for the specific form of zero queueing delay. Simply make reference to equation (1) instead.

{\color{blue}\noindent\textbf{Response.}
We have made a reference to equation (1).  But we do have a slight preference to keep the expression since we wanted the model section to be relatively self-contained.  We have changed it from on display to in line to minimize the space needed.  Please see Page~6. 
}

Punctuation is missing after some of the equations. E.g., equation (13).

{\color{blue}\noindent\textbf{Response.}
Fixed.  Please see equation (14) on Page~11.
}



==> Achieving Zero Queueing Delay for Parallel Jobs/simulation-old.tex <==
% simulation results when scale up N
% figure: x-axis: N
% y axis: delay/max{task delays}
% curves: different d's
% address the comment that zero queueing delay can be achieved with reasonable values of k and N
% explore the threshold of d for zero queueing delay

% comparison with non-parallel setting

{\color{blue}
In this section, we perform three sets of simulations to demonstrate our theoretical results and explore settings beyond those in our theoretical analysis.  The first set illustrates the scaling behavior of the system as $N$ grows under various probe ratios, and investigates the gap between our achievability results and impossibility results.  The second set looks into the effect of parallelization by comparing our setting with a setting where the tasks of a job cannot be executed in parallel. Finally, the third set experiments on more general service time distributions beyond the exponential distribution.


\subsection{Scaling Behavior with Various Probe Ratios}\label{subsec:scaling}
This set of simulations use the setting of our theoretical results with $\lambda=1-N^{-0.3}$ ($\alpha=0.3$ and $\beta=1$). We let $k$, the number of tasks per job, scale with $N$ as $k = \lfloor \ln^2 N \rfloor$.  The values for $N$ and the corresponding $k$ used in the simulations are given in Table~\ref{table:scale-system}. These values are reasonable in practice considering that datacenters nowadays typically have tens of thousands of nodes (each with multiple cores) per cluster and a job may consist of hundreds of tasks \cite{amvrosiadis_2018}.

%In this simulation, we follow the setting of our basic model. Jobs arrive in a Poisson process with arrival rate $ \frac{N(1-N^{-0.3})}{k}$, so $\alpha = 0.3$ here. Each job contains $k$ parallel sub-tasks whose service time independently follows a  exponential distribution with mean $1$. Jobs are scheduled using batch-filling algorithm. Twelve scales of systems are considered as per Table \ref{table:scale-system} where $k = \lfloor \ln^2 N \rfloor.$
% \begin{table}[!hbp]
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% $N$ & 32   & 64   & 128  & 256   & 512   & 1024  \\ \hline
% $k$ & 12   & 17   & 23   & 30    & 38    & 48    \\ \hline
% $N$ & 2048 & 4096 & 8192 & 16384 & 32768 & 65536 \\ \hline
% $k$ & 58   & 69   & 81   & 94    & 108   & 122   \\ \hline
% \end{tabular}
% \caption{Scaling of the System}
% \label{table:scale-system}
% \end{table}
\begin{figure}[!hbp]
\begin{minipage}[c]{.4\textwidth}
\centering
\begin{tabular}{r r r r r}
\\
\toprule
$N$ & 32   & 64   & 128  & 256   \\
$k$ & 12   & 17   & 23   & 30    \\
\midrule
$N$ & 512   & 1024  & 2048 & 4096 \\
$k$ & 38    & 48    & 58   & 69 \\
\midrule
$N$  & 8192 & 16384 & 32768 & 65536 \\
$k$  & 81   & 94    & 108   & 122   \\
\bottomrule\\
\end{tabular}
\captionof{table}{Scaling parameters.}
\label{table:scale-system}
\end{minipage}
\hspace{0.3in}
\begin{minipage}[c]{.5\textwidth}
\centering
\scalebox{0.32}{\input{picture/diff-d.pgf}}
\vspace{-0.1in}
\caption{Queueing delays under different probe ratios: $d_1$ is sufficient for convergence to zero queueing delay; $d_1>d_4>d_3>d_2$.}
\label{fig:different-d}
\end{minipage}
\vspace{-0.2in}
\end{figure}


We explore four scaling settings of the probe ratio.  The first setting uses a probe ratio of $d_1 = \frac{4}{(1-\lambda)h}=\frac{4N^{\alpha}}{h}$ with $h = \lceil\frac{\log k}{\log \log k} \rceil$, which satisfies the conditions in Theorems~\ref{main_theorem_1} and \ref{theorem zero delay} to achieve zero queueing delay.  The second setting uses a probe ratio of $d_2 = \exp{(0.5\log N / \log k)}$, which is slightly larger than the value in Theorems~\ref{main_theorem_2} and \ref{theorem lower d} that guarantees non-zero queueing delay.  The other two settings use probe ratio values $d_3$ and $d_4$ that interpolate between $d_1$ and $d_2$ to investigate the threshold under which the system transits from zero queueing delay to non-zero queueing delay.  Note that $d_1>d_4>d_3>d_2$ for all values of $N$ in the simulations. More details of the settings can be found in Appendix~\ref{sec:experiment}.

Figure~\ref{fig:different-d} shows the simulation results for the queueing delay $\frac{\expect[T-T^*]}{\expect[T^*]}$.  The curve for $d_1$ demonstrates the trend for the queueing delay to converge to zero as predicted by the theoretical results.  It does not exactly reach zero but becomes reasonably close. Under the probe ratios $d_2$ and $d_3$, the queueing delay clearly deviates from zero.  Under the probe ratio $d_4$, the queueing delay flattens out after some initial drop as $N$ becomes large.  Therefore, it is plausible that the transition from zero queueing delay to non-zero queueing delay happens at a probe ratio value near $d_4$.  Since $d_4$ is much closer to $d_1$ than to $d_2$, we expect our impossibility results to be not tight.  Pinning down the exact threshold for the transition (or proving the nonexistence of such a threshold) is of great theoretical interest and we leave it for future research.

%Let $h = \lceil\frac{\log k}{\log \log k} \rceil$. We set $d_1 = \frac{4}{(1-\lambda)h},d_2 = e^{0.5\log N / \log K}$ as per Theorem \ref{theorem zero delay} and Theorem \ref{theorem lower d}. Besides, two other scalings of the probe ratio, $d_3 = d_2 + \sqrt{d_1}$ and $d_4 = d_2 + d_1^{7/8}$, are studied for a sharper threshold to achieve zero queueing delay. We refer the reader to Appendix \ref{sec:experiment} for a detailed setting. The value of $\frac{\expect[T]}{\expect[T^*]}$ , which we call relative job delays, is shown in Figure \ref{fig:different-d}.
% \begin{figure}
% \begin{minipage}[t]{.45\textwidth}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% $N$ & 32   & 64   & 128  & 256   \\ \hline
% $k$ & 12   & 17   & 23   & 30    \\ \hline
% $N$ & 512   & 1024  & 2048 & 4096 \\ \hline
% $k$ & 38    & 48    & 58   & 69 \\ \hline
% $N$  & 8192 & 16384 & 32768 & 65536 \\ \hline
% $k$  & 81   & 94    & 108   & 122   \\ \hline
% \end{tabular}
% \captionof{table}{Scaling of the system}
% \label{table:scale-system}
% \end{minipage}
% \hspace{0.3in}
% \begin{minipage}[t]{.45\textwidth}
% \centering
% \scalebox{0.32}{\input{picture/diff-d.pgf}}
% \caption{Relative job delays under different probe ratios. Here $d_1$ is the proved sufficient probe ratio to achieve zero queueing delay; $d_2$ is the proved necessary probe ratio; $d_3,d_4$ are two intermediate probe ratios.}
% \label{fig:different-d}
% \end{minipage}
% \end{figure}
%Figure \ref{fig:different-d} verifies our theory that the probe ratio $d_1$ leads to asymptotic zero queueing delay while the probe ratio $d_2$ always results in non-negligible delays. However, Figure \ref{fig:different-d} also indicates that the sharp lower bound may indeed be close to the upper bound $d_1$, which we leave for future research.  


\subsection{Effect of Parallelization}
This set of simulations demonstrates how parallelization plays a critical role in reducing the probe overhead needed for achieving zero queueing delay.  Towards this end, we simulate a system where the parallel structure of jobs is taken away.  In particular, each job in this non-parallel model is indivisible with an exponentially distributed service time with mean equal to $k$ (denoted as $\text{Exp}(1/k)$). The queueing delay for such non-parallel jobs is defined with respect to $T^*\sim\text{Exp}(1/k)$, which is the job delay without queueing.  Figure~\ref{fig:non-parallel} shows that the probe overhead that yields zero queueing delay for parallel jobs is no longer sufficient for achieving zero queueing delay for such non-parallel jobs.
% needs to confirm probe overhead

%We next compare our result with the non-parallel setting. To be specific, this simulation follows the same setting as in the last one. But in addition to parallel jobs, we consider non-parallel jobs where each job only contains one task whose service time is exponentially distributed with mean $k$. Then every parallel and non-parallel job shares the same expected total amount of work equal to $k$. To study the benefit of a parallel structure, we compare the relative delays of parallel and non-parallel jobs using the same probe ratio $d_1$. Results are shown in Figure \ref{fig:non-parallel}.
\begin{figure}
\begin{minipage}[t]{.45\textwidth}
    \centering
    \scalebox{0.32}{\input{picture/nonparallel-comparison.pgf}}
    \vspace{-0.1in}
    \caption{Effect of parallelization on queueing delays.}
\label{fig:non-parallel}
\end{minipage}
\hspace{0.3in}
\begin{minipage}[t]{.45\textwidth}
    \centering
    \scalebox{0.32}{\input{picture/diff-dist.pgf}}
    \vspace{-0.1in}
    \caption{Queueing delays under different service time distributions.}
    \label{fig:different-dist}
\end{minipage}
\vspace{-0.2in}
\end{figure}

\subsection{More General Distributions for Task Service Times}
The last set of simulations explore distributions beyond the exponential distribution for task service times.  Figure~\ref{fig:different-dist} shows the results for three distributions: (1) \emph{Exponential distribution} with rate $1$ ($\text{Exp}(1)$).  This is the baseline distribution that is assumed for our theoretical analysis. (2) \emph{Bounded Pareto} in range $[1,1000]$ with a shape constant $1.5$. (3) \emph{Hyper-exponential} that follows $\text{Exp}(1)$ with probability $0.99$ and $\text{Exp}(0.01)$ with probability $0.01$.  We re-scale the arrival rates so all the systems have the same load $\lambda=1-N^{-0.3}$.  The probe overhead is chosen to be the $d_1$ in Section~\ref{subsec:scaling} such that zero queueing delay is provably achievable under the exponential distribution. 

We observe that empirically, the queueing delay has a trend that approaches zero under all the three distributions, although the latter two distributions have larger coefficients of variation than the exponential.  These simulation results suggest that our theoretical results have some robustness with respect to service time distributions.  We comment that there is little existing work on zero queueing delay for general service time distributions with the exception of \cite{b5}, which studies the Coxian-2 distribution for non-parallel jobs.  Generalizing our analysis to general service time distributions is a research direction that deserves much further effort, as it is for many problems in queueing systems.


%The last simulation generalizes the parallel-job model to different service time distributions for tasks. Denote the service time of a task by $S$. In particular, we consider the following three distributions: 1) \textbf{Exp(1)}, the service time follows a exponential distribution with mean $1$; 2) \textbf{Bounded Pareto}, the task service time $S$ is sampled from a bounded Pareto distribution in range $[1,1000]$ with the shape constant $1.5$; 3) \textbf{Hyper-exponential}, the service time $S$ follows Exp(1) with probability $0.99$, and follows Exp(0.01) with probability $0.01$. Note that in the simulation, the arrival rate of jobs is set as $\frac{N(1-N^{-0.3})}{k\expect[S]}.$ To study the effect of service time distribution, we fix the probe ratio as $d_1$ for all three distributions. Figure \ref{fig:different-dist} then shows how the convergence of relative delays is related to the service time distribution.

%For both the hyper-exponential distribution and the bounded Pareto distribution, our reduced probe ratio is feasible to (asymptotically) achieve zero queueing delay.
}


==> Achieving Zero Queueing Delay for Parallel Jobs/simulation.tex <==

{
In this section, we perform two sets of simulations to demonstrate our theoretical results and explore settings beyond those in our theoretical analysis.  The first set illustrates the scaling behavior of the system as $N$ grows under various probe ratios, and investigates the gap between our achievability results and impossibility results.  The second set of simulations experiment on more general service time distributions beyond the exponential distribution and correlation among task service times. 


%{
%Note that for each plot, we repeat the simulation for ten runs and show the averaged value. Nevertheless, error bars in each plot is insensible since results are almost the same in each run. We provide exact values of curves and errors in Appendix~\ref{sec:exactval}.}


\subsection{Scaling Behavior with Various Probe Ratios}\label{subsec:scaling}
This set of simulations use the setting of our theoretical results with $\lambda=1-N^{-0.3}$ ($\alpha=0.3$ and $\beta=1$). We let $k$, the number of tasks per job, scale with $N$ as $k = \lfloor \ln^2 N \rfloor$.  The values for $N$ and the corresponding $k$ used in the simulations are given in Table~\ref{table:scale-system}. These values are reasonable in practice considering that datacenters nowadays typically have tens of thousands of nodes (each with multiple cores) per cluster and a job may consist of hundreds of tasks \cite{amvrosiadis_2018}.


\begin{table}[!hbp]
\begin{tabular}{r r r r r r r r r r r r r}
\toprule
$N$ & 32   & 64   & 128  & 256   & 512   & 1024  & 2048 & 4096 & 8192 & 16384 & 32768 & 65536 \\ 
$k$ & 12   & 17   & 23   & 30    & 38    & 48   & 58   & 69   & 81   & 94    & 108   & 122   \\
\bottomrule
\end{tabular}
\caption{Scaling parameters}
\label{table:scale-system}
\vspace{-0.2in}
\end{table}


\begin{figure}
\begin{minipage}[t]{.45\textwidth}
\centering
\scalebox{0.32}{\input{picture/diff-d.pgf}}
\vspace{-0.2in}
\caption{Queueing delays under different probe ratios: $d_1$ is sufficient for convergence to zero queueing delay; $d_1>d_4>d_3>d_2$.}
\label{fig:different-d}
\end{minipage}
\hspace{0.3in}
\begin{minipage}[t]{.45\textwidth}
    \centering
    \scalebox{0.32}{\input{picture/diff-dist.pgf}}
    \vspace{-0.2in}
    \caption{Queueing delays under different service time distributions.}
    \label{fig:different-dist}
\end{minipage}
\vspace{-0.1in}
\end{figure}


We explore four scaling settings of the probe ratio.  The first setting uses a probe ratio of $d_1 = \frac{4}{(1-\lambda)h}=\frac{4N^{\alpha}}{h}$ with $h = \lceil\frac{\log k}{\log \log k} \rceil$, which satisfies the conditions in Theorems~\ref{main_theorem_1} and \ref{theorem zero delay} to achieve zero queueing delay.  The second setting uses a probe ratio of $d_2 = \exp{(0.5\log N / \log k)}$, which is slightly larger than the value in Theorems~\ref{main_theorem_2} and \ref{theorem lower d} that guarantees non-zero queueing delay.  The other two settings use probe ratio values $d_3$ and $d_4$ that interpolate between $d_1$ and $d_2$ to investigate the threshold under which the system transits from zero queueing delay to non-zero queueing delay.  Note that $d_1>d_4>d_3>d_2$ for all values of $N$ in the simulations. More details of the settings can be found in Appendix~\ref{sec:experiment}.

Figure~\ref{fig:different-d} shows the simulation results for the queueing delay $\frac{\expect[T-T^*]}{\expect[T^*]}$, 
{ where the results are averaged over ten independent runs.  Please refer to Appendix~\ref{sec:exactval} for the exact values and standard deviations.  Since the standard deviations are very small ($\sim 10^{-4}$), the error bars are not visible in the plots.
}
The curve for $d_1$ demonstrates the trend for the queueing delay to converge to zero as predicted by the theoretical results.  It does not exactly reach zero but becomes reasonably close. Under the probe ratios $d_2$ and $d_3$, the queueing delay clearly deviates from zero.  Under the probe ratio $d_4$, the queueing delay flattens out after some initial drop as $N$ becomes large.  Therefore, it is plausible that the transition from zero queueing delay to non-zero queueing delay happens at a probe ratio value near $d_4$.  Since $d_4$ is much closer to $d_1$ than to $d_2$, we expect our impossibility results to be not tight.  Pinning down the exact threshold for the transition (or proving the nonexistence of such a threshold) is of great theoretical interest and we leave it for future research.


{
To further investigate how $k$, the number of tasks per job, affects the scaling behavior under different probe ratios, we examine another setting where $k = \lfloor \sqrt{N} \rfloor$.  This scaling of $k$ is beyond our theoretical framework, but the queueing delays exhibit similar trends as those in the setting where $k = \lfloor \ln^2 N \rfloor$.  Details of the simulation results are given in Appendix~\ref{sec:newk}.}


{
\subsection{More General Settings for Task Service Times}
This set of simulations explore distributions beyond the exponential distribution for task service times and correlation among their service times.  Figure~\ref{fig:different-dist} shows the results for four settings: (1)~\emph{i.i.d.\ exponential distribution} with rate $1$ (denoted as $\text{Exp}(1)$).  This is the baseline distribution that is assumed for our theoretical analysis. (2)~\emph{i.i.d.\ bounded Pareto} in range $[1,1000]$ with a shape constant $1.5$. (3)~\emph{i.i.d.\ hyper-exponential} that follows $\text{Exp}(1)$ with probability $0.99$ and $\text{Exp}(0.01)$ with probability $0.01$.  We re-scale the arrival rates so all the systems have the same load $\lambda=1-N^{-0.3}$.
(4)~\emph{S\&X model} for correlated task service times, which is a model proposed in \cite{GarHarSch_16} and has been extensively studied since then.  In the S\&X model, the service time of the each task in a job can be written as $S\cdot X$, where every task in the same job shares the same $X$, but different tasks have their own $S$'s that are independent among tasks. Here we assume $S$ and $X$ are both exponentially distributed with rate $1$.} The probe overhead is chosen to be the $d_1$ in Section~\ref{subsec:scaling} such that zero queueing delay is provably achievable under the exponential distribution. 

{
We observe that empirically, the queueing delay has a trend that approaches zero under all the four settings, despite of the larger coefficients of variation for the bounded Pareto and hyper-exponential distributions and the correlation among task service times in the S\&X model.  These simulation results suggest that our theoretical results have some robustness with respect to service time distributions and correlations.  We comment that there is little existing work on zero queueing delay for general service time distributions with the exception of \cite{b5}, which studies the Coxian-2 distribution for non-parallel jobs.  Generalizing our analysis to general service time distributions with possible correlations is a research direction that deserves much further effort, as it is for many problems in queueing systems.}
}


==> response-letter.tex <==

{\color{blue}
We would like to thank the reviewers and the TPC chairs for the constructive comments and suggestions.  We have carefully revised our paper to address the one-shot revision requirements and the individual comments from the reviewers.  Some key highlights of the changes are summarized below:
\begin{itemize}[leftmargin=1em]
    \item We have conducted simulation experiments based on the suggestions of the reviewers and added Section~7 to present the results.  Through the simulations, we are able to demonstrate the consistency between numerical results and our theoretical results under reasonable settings, and to address some gaps in the theoretical analysis.
    \item We have added Section~6 to discuss the more stringent notion of zero queueing delay mentioned by the reviewers that requires all the tasks of a job to have zero waiting time in queues.
    \item We have made major adjustments to the structure of the paper to make the proofs of the main results more accessible.  These adjustments include developing more understanding of zero queueing delay on a job level at the beginning of Section~4, sketching the proofs before presenting the formal proofs in Sections~4 and 5, and moving lemmas and their proofs to the appendix.
    \item We have added many intuitions, explanations, clarifications, and justifications throughout the paper.
\end{itemize}

Below we first give our detailed responses to the one-shot revision requirements.  Then we will address the individual comments of each of the reviewers, focusing more on the comments that are not addressed in our responses to the one-shot revision requirements.  Our responses are in blue and the quoted requirements/comments are in black.  We also highlighted major changes in the paper in blue text.}


\section*{One-Shot Revision Requirements}

The one-shot revision requires the authors to address all the comments in each of the reviews and to add a detailed set of numerical experiments that address the important points below. Acceptance is contingent on the authors making these required changes.

In addressing all the reviewer comments, the authors must specifically address the following points:
{\color{blue} (We have added a prefix ``I.'' to the indices of the comments for ease of reference.)}
\begin{enumerate}[label=\textbf{(I.\alph*)},leftmargin=2.1em]
    \item The presentation and structure of the paper needs to be improved. Some or all of the proofs should be deferred to an appendix, and instead in the main body of the paper the authors could provide a sketch of the proof (or a high-level explanation) and provide more insights on the performance. The extra space should be devoted for a numerical section.
    
    {\color{blue} We have made the following major adjustments to the structure of the paper to improve the presentation based on the comments and suggestions of the reviewers:
    \begin{itemize}[leftmargin=1em]
        \item For proving the achievability results, we have added three segments at the beginning of Section~4 (Pages 8--10) to develop more understanding on how zero queueing delay relates to the system state, and to provide a proof sketch.  We have then moved an additional lemma and the proofs of all the lemmas involved to Appendix~A.  However, the proofs of Theorems~3.1 and 3.2 remain in this section since we deem them as essential for understanding the theoretical results of the paper, which constitute a main part of the contributions of the paper.
        
        \item For proving the impossibility results, we have added a proof sketch at the beginning of Section~5 (Page~16) to help guide the readers through the proofs.  Again, we have moved the lemmas and their proofs to Appendix~B, but have kept the proofs of Theorems~3.3 and 3.4.  The proof techniques for Theorem~3.3 are novel and we believe that they could be of interest to many readers.
        
        \item As we summarized at the beginning of this response letter, we have added simulation results (Section~7) and discussion on another notion of zero queueing delay (Section~6), and have made an effort to provide insights by integrating many intuitions, explanations, clarifications, and justifications throughout the paper.  More details can be found in our responses to other revision requirements.
    \end{itemize}
    }
    
    \item The notation used in the paper should be defined.
    
    {\color{blue} We have added a paragraph as a reminder to Bachmann--Landau asymptotic notation in Section~1 right before the related work subsection (Page~4).  We have also added clarifications on the definition of the generator of the fluid model in Section~4.1 (Page~10).  %%Other notation missing?
    }
    
    \item The paper claims that their modeling assumptions are more realistic than those previously considered in the literature. This claim needs to be better substantiated. The authors should carefully justify their model providing examples in which the model can be applied. 
    
    {\color{blue}
    We address this comment for the following modeling assumptions.
    \begin{itemize}[leftmargin=1em]
        \item The main modeling assumption that differentiates our paper from papers in the literature is the parallel job assumption, i.e., we assume that each job can be parallelized into multiple tasks.  This assumption reflects the widely adopted parallel computing framework in many applications.  We have added more references in Section~1 (Page~2) to justify the predominance of such a model and to give application examples (distributed cloud computing, distributed file systems, machine learning systems).
        
        For such a model with parallel jobs, we need to choose the performance metric properly.  In this paper, we focus on the delay of jobs rather than the delay of tasks since usually a job is a meaningful unit for users.  Our choice is in line with the design goal of many practical schedulers (examples given in Section~1 on Page~2).
        
        However, despite the popularity of parallelism in practice, there is a significant gap in the literature of queueing theory/stochastic systems, where jobs that can be parallelized have not been extensively studied.  There is very limited amount of prior work that considers parallel jobs and analyzes job delay, and the very few papers that do analyze job delay have only got fluid-level optimality at the best and have only considered a constant load.
        We have added a bit more emphasis on this when discussing the challenges and our results in Section~1 (before the reminder of Bachmann-Landau notation on Page~4).
        
        \item Another modeling assumption we make is that the task service times are i.i.d.\ exponential.  We would like to clarify that we did not claim that this modeling assumption is more realistic than those previously considered, since it is a rather typical assumption made in theoretical studies.  However, we are able to use simulations to empirically
        investigate how the service time distribution affects the trend of queueing delay.  We have added simulations in Section~7.2 to experiment on hyper-exponential distributions and bounded Pareto distributions as distributions for task service times.  The simulation results show that the queueing delay also has a trend to converge to zero under these two distributions.  We leave the theoretical analysis under these distributions and also correlated service times as future research directions.
        
        \item We assume that $k$, the number of tasks in a job, scales with $N$, the number of servers.  The motivation for this modeling assumption is to capture the increasing size of jobs as the computing power grows.  We have added some clarifications throughout the paper to make this assumption even more explicit.  Since studies on parallel jobs are scarce, it is hard to conclude if this assumption is more realistic than those in existing work or not.  In fact, we hope that our paper can serve as a first step towards characterizing behaviors under different scaling regimes.
        
    \end{itemize}
    }
    
    \item The paper considers a specific form of zero queueing delay that actually allows tasks in a job to wait in queues for non-negligible amounts of time. The paper should mention other possible forms of zero queueing delay that are more stringent, and discuss how the analysis presented in the paper might be extended to address these more stringent forms of zero queueing delay.
    
    {\color{blue}
    We have added a section (Section~6, Page~19) to discuss the more stringent notion where all the tasks of a job need to be assigned to idle servers.  We show an impossibility result that this more stringent notion cannot be achieved when the probe overhead is $O(\frac{1}{1-\lambda})$.  However, we wanted to point out that although this notion seems to be similar to the notion of zero queueing for non-parallel (single-task) jobs, the two systems have fundamentally different dynamics and thus it is hard to make an analogy.  We would like to also argue that the notion we proposed that compares the actual job delay with the hypothetical job delay assuming no queueing is more natural and thus remains the focus of the paper.  As we explained in the first bullet point above, performance on a job level is what the users care the most, and this is reflected in the design goal of many practical schedulers.  We also address the comparison with single-task setting in the comment (I.e) below. 
    }
    
    \item  One of the main claims of the paper is that thanks to parallelization, asymptotic zero queueing delay is obtained with lower overhead than in the single-task setting. However, the performance metric is looser than in the related literature, where typically the waiting time is shown to be $0$ asymptotically, and hence the comparison is not fair. This needs to be clearly explained throughout the paper. In addition, the revision should address this issue and provide evidence that parallelization will also achieve $0$ waiting time asymptotically (all tasks should find an empty server, except those that are not the head-of-the-line in the batch). In order to achieve this, the revision should carry out the analysis of the parallelization scheme for the waiting time.
    
    {\color{blue}
    First, we would like to clarify that it is hard to conclude that our notion of zero queueing delay is looser than in the related literature since the majority of existing work considers non-parallel (single-task) jobs.  We have added explanations on how a system with parallel jobs has fundamentally different dynamics from a system with non-parallel jobs (paragraphs under ``Challenges and our results'' in Section~1 on Page~3, Section~6).  We have also added clarifications on how our notion is different from the conventional notion for non parallel jobs (blue paragraph at the top of Page~3).
    
    We respectfully disagree that parallelization needs to necessarily guarantee that all tasks find empty servers.  As we argued in the response to comment (I.c) above, it is much more typical that users consider performance on a job level.
    
    We wanted to add that we may be able to address this comment better if the reviewers can clarify what they refer to as tasks ``that are not the head-of-the-line in the batch.''  Tasks of the same job arrive together and there is no particular ordering among them.
    }
\end{enumerate}

The authors must conduct numerical experiments whose results confirm and demonstrate all the claims of the paper based on the asymptotic results for realistic parameter values. Of particular importance for parameter values is the number of parallel tasks $k$ and showing that all the claims of the paper hold for moderately large values of $k$. In addition, the authors must conduct corresponding numerical experiments for increasingly larger values of $k$ and $N$ to demonstrate how these numerical results approach the asymptotic results and to provide an understanding of the convergence behavior toward the asymptotic results. In conducting these numerical experiments, it is of particular interest for the authors to address the following points:
{\color{blue} (We have added a prefix ``II.'' to the indices of the comments for ease of reference.)}
\begin{enumerate}[label=\textbf{(II.\alph*)},leftmargin=2.6em]
\item One of the main claims of the paper is that thanks to parallelization, asymptotic zero queueing delay is obtained with lower overhead than in the single-task setting. However, the performance metric is looser than in the related literature, where typically the waiting time is shown to be $0$ asymptotically, and hence the comparison is not fair. If it is not possible to carry out the analysis of the parallelization scheme to achieve $0$ waiting time asymptotically (all tasks should find an empty server, except those that are not the head-of-the-line in the batch) as noted above, then the paper should explain the reasons for this and the numerical experiments should assess whether parallelization also achieves asymptotically $0$ waiting delay, and if it does, further assess the overhead required for it.

{\color{blue}Please refer to our responses to comments (I.d) and (I.e) in the last group of comments.  Since we feel that we have addressed this concern sufficiently, we did not perform further numerical experiments.
}

\item There seems to be a gap between the regimes in which the asymptotic relative delay vanishes, and when it doesn't. As parameters such as $k$ and $N$ are increased, the numerical experiments should investigate this gap. As parameters such as $k$ and $N$ are increased, the numerical experiments should investigate the gap in the bounds and provide an understanding of the convergence behavior toward the asymptotic results.

{\color{blue}
We thank the reviewers for this great suggestion.  We have added simulation experiments for different scalings of the probe ratio $d$ to investigate this gap.  Please see Section~7.1 on Pages~19--20 for the details.  A quick summary is that for a probe ratio that satisfies the conditions for achievability (Theorems~3.1 and 3.2), the empirically trend of queueing delay is consistent with the theoretical results; the simulation results suggest that our impossibility results are not tight, which causes the gap.  These simulation results serve as great guidelines for future research directions.
}

\item With the unfair queueing delay comparison, the total service requirement of a job being smaller than its original size and other differences between the single-task and parallel-tasks setting (see reviewer comments), it is important to pinpoint the main reasons for the differences in the asymptotic behavior. The numerical experiments should investigate and identify the main reasons for these differences.

{\color{blue}
For whether our notion of zero queueing delay induces fair comparisons, please refer to our responses to comments (I.d) and (I.e) in the last group of comments.

We would like to make some clarifications regarding the concern related to the total service requirement.  When a job is parallelized, its total size is not altered, but the job can be served by multiple servers simultaneously in parallel.  We agree that when there is no queueing, the job delay after parallelization becomes smaller than that in the case of no parallelization, which is the motivation for parallelization.  Our notion of zero queueing delay is relative to the job delay under parallelization, which should not cause unfairness towards our favor in our opinion.

We would like to argue that this reduction in probe overhead reflects the overall effect of parallelization on the system.
There are several factors at play that are brought by parallelization all together.  This makes it hard to quantify their individual effects through numerical experiments since it is hard if not impossible to take away one factor without affecting other factors.

We list those factors below.  First, for tasks of the same job, the probe overhead quota is pooled together and their assignment is coordinated, leading to a more effective use of the state information.  Second, a job with parallel tasks can better tolerate task delays since the job delay is anyway determined by the slowest task.  Furthermore, work arrives to the system in a more bursty fashion under parallelization due to the batch effect.

We have added this discussion in the ``Challenges and our results'' subsection of Section~1 on Pages~3--4.
}


\item Include a discussion of the comparison between the numerical results and theoretical results and an understanding that is provided by this comparison.

{\color{blue} We have included such discussions throughout the added section for simulation results (Section~7).
}

\end{enumerate}


It is important to emphasize that acceptance is contingent on the numerical experiments confirming and demonstrating all the claims of the paper based on the asymptotic results for realistic parameter values and demonstrating how these numerical results approach the asymptotic results for increasingly larger values of these parameter values.

{\color{blue} We thank the reviewers again for the suggestions on numerical experiments.  We found the comparisons of theoretical results and simulation results very inspiring.  We hope that the readers will be able to gain more understanding and insights from this added section.
}


\section*{Reviewers' Comments}

\subsection*{Review \#67A}
\textbf{Paper summary}

This paper studies a queueing system with $N$ servers in which upon arrival of a job, $d$ servers are probed, and $k <d$ tasks of the job are dispatched to the servers with shortest queue-lengths. A job is completed when all of its $k$ tasks finish service. In an asymptotic regime in which $k$, $d$, and $N$ tend to infinity, the paper shows that under suitable choice of $d$ and $k$, the relative difference between the obtained delay and the minimum achievable one tends to $0$. 

The theoretical contribution is sound, but not a breakthrough in the light of recent papers that have obtained results of similar nature. The paper lacks a numerical section, and in my view, the theoretical contribution in itself is not significant enough to warrant publication in Sigmetrics.

{\color{blue} \noindent\textbf{Response.}
We have added explanations on how a system with parallel jobs has fundamentally different dynamics from a system with non-parallel jobs and why that makes the analysis more challenging.  Please refer to the ``Challenges and our results'' subsection of Section~1 on Pages~3--4 for more details.  We have added a numerical section as Section~7.  Please refer to the responses to the one-shot revision requirements and Section~7 on Pages~19--20 of the paper for more details.
}

\noindent\textbf{What are the strengths of the paper?}

Sound theoretical analysis of a model of practical interest.

\noindent\textbf{What area of the paper need improvement?}

A numerical section would have been appreciated provide more insights into the performance of the system. See details below.

{\color{blue} \noindent\textbf{Response.}  Please refer to our responses to the one-shot revision requirements for discussions on the numerical section.}

The presentation could be improved. For example, asymptotic notation is extensively used, little-o, big-O, $\omega$, $\Omega$, without ever being defined. The fact that $k$ and $d$ scale with $N$ should also made clear from the abstract on.

{\color{blue} \noindent\textbf{Response.}  We have added a paragraph as a reminder to Bachmann--Landau asymptotic notation in Section~1 right before the related work subsection (Page~4).  We have also made the fact that $k$ and $d$ scale with $N$ more explicit in the abstract and throughout the paper.
}

One of the main messages of the paper is that by parallelizing, zero queueing delay can be obtained with less overhead than in the single-task setting. However, the modeling assumptions are typically different, and as a consequence, it is not obvious to conclude that parallelizing improves the asymptotic performance. This should be explained clearly throughout.

{\color{blue} \noindent\textbf{Response.} 
Please refer to our responses to the one-shot revision requirements (I.d), (I.e) and (II.c).}



\noindent\textbf{Other comments for author}

There seems to be a gap between the regimes in which the asymptotic relative delay vanishes, and when it doesn't. This gap could have been explored numerically.

{\color{blue} \noindent\textbf{Response.}  We thank the reviewer for this great suggestion!  We have added Section~7.1 on Pages~19--20 to investigate this gap.  Please refer to our response to the one-shot revision requirement (II.b).}

The model assumes iid service times (exponential distribution) for the tasks. If the original service time of a job is 1, then the maximum of $k$ independent tasks with each a mean service requirement of $1/k$ is smaller than 1, i.e., the mean service requirement with multiple tasks is smaller than the original one. This assumption plays a key role in the analysis, and its impact could have been explored numerically, for example assuming non-exponential service times, identical copies across tasks, other correlation structure among the service times of tasks etc.

{\color{blue} \noindent\textbf{Response.}  We have added Section~7.2 (Page~20) to explore non-exponential service times.  Please also refer to the second bullet point in our response to the one-shot revision requirement (I.c).

We would like to clarify that we normalize the mean task size to be $1$.  The parallelization does affect the job delay even under no queueing.  But we believe that it does not cause unfairness towards our favor since our notion of zero queueing delay is relative to the job delay under parallelization.  Please also refer to our response to the one-shot revision requirement (II.c).
}

In papers considering the single-task case the main criteria is that the waiting probability tends to $0$, whereas in the present paper the relative delay is considered. In addition, the total service requirement of a job is smaller than its original size. It is therefore not clear to pinpoint the main reason for the difference for the difference in the asymptotic behavior. The comparison with related literature is not carried out on the same ground. This is also that could  have been further explored numerically.

{\color{blue} \noindent\textbf{Response.}  Please refer to our responses to the one-shot revision requirement (I.d), (I.e) and (II.c) for the discussions on the comparison with non-parallel models.}

The paper claims that the modeling assumptions considered (multiple tasks, iid distributed, with $d$ and $k$ scaling with $N$) are more realistic than the ones considered in previous literature. A reference is needed to support this claim, otherwise the claim should be downplayed.

{\color{blue} \noindent\textbf{Response.}  Please refer to our response to the one-shot revision requirement (I.c) for justifications of some of our modeling assumptions.
}

From Section 4.1 on, what is the generator of a fluid model? 

{\color{blue} \noindent\textbf{Response.}   We have added clarifications on the definition of the generator of the fluid model in Section~4.1 (Page~10).}

\noindent Other comments:

- Section 2, 8th line, ``when all of ITS tasks finish...''

{\color{blue} \noindent\textbf{Response.}  Fixed. Please see Page~5.}

- After eq (5). "Therefore, the batch-filling policy achieves 0 queueing delay". Is this concluded from THM 3.2, or THM 3.1? Be more specific.

{\color{blue} \noindent\textbf{Response.}  It is from Theorem~3.2.  We have made it more specific on Page~7.}




\subsection*{Review \#67B}
\noindent\textbf{Paper summary}

This paper considers a classical load balance architecture with one dispatcher and $N$ parallel homogeneous servers. Jobs arrive at the system according to a Poisson process.  Differently from the classical case jobs are not atomic objects. They can be break in $k$ tasks, which can be executed in parallel (of course, a job finishes upon the completion of the  last task). 

Authors propose  batch-filling policy, a variant of the classical Po-d (Power of d) policy, and show that  it achieves asymptotically zero queuing delay (i.e. the sojourn time of a job in the system is asymptotically dominated by its service time) as long as d is consistently chosen.


\noindent\textbf{What are the strengths of the paper?}

The paper  seems technically sound (even if I could not check completely).  Form a technical point of view results are non trivial. Even is the topic is well established, it is still a relevant topic, and any results that advances  this field can be of interest.


\noindent\textbf{What area of the paper need improvement?}

The assumption that jobs breaks into tasks that can be executed in parallel should be better motivated. For example this is true in Hadoop if reduce tasks are ignored, but can we  really ignore them?

{\color{blue}\noindent\textbf{Response.}
We thank the reviewer for this great suggestion!
We have added more references in Section~1 (Page~2) to justify the predominance of such a model and to give application examples (distributed cloud computing, distributed file systems, machine learning systems).

We agree that the reduce tasks cannot be really ignored in Hadoop.  However, we would like to think that our analysis can be applied to study the completion time of the map phase, which can provide a good basis for further analysis on the overall delay.  More generally, we hope that our analysis can contribute towards understanding parallel jobs with more complicated structures such as multiple stages or more general precedence relationship among tasks.
}

\noindent\textbf{Other comments for author}

I think the authors should carefully justify their model providing examples in which  their model can be applied. For the rest the paper is pretty well written (even if it is not an easy read). I have appreciated the attempt made by the authors to provide a high-level overview of the proofs  (at least for what concerns the upper-bound) before  digging deeply into details.

{\color{blue}\noindent\textbf{Response.} We thank the reviewer for appreciating our attempt to make the proofs more accessible.  We have made further changes towards this goal.  Please refer to our response to the one-shot revision requirement (I.a).
}






\subsection*{Review \#67C}
\noindent\textbf{Paper summary}

This paper revisits the well-studied problem of achieving zero asymptotic queueing delay using the power-of-d choices policy by replacing single indivisible jobs with jobs consisting of parallel tasks. The paper shows that a previously proposed variant of the power-of-d-choices policy in the literature achieves zero asymptotic queueing delay with a probe overhead for d that is an improvement over previous studies and includes the number of tasks in each job.


\noindent\textbf{What are the strengths of the paper?}

The paper revisits an important load balancing problem with the extension to parallel jobs. Theoretical results are established that support zero queueing delays for larger values of probe overhead d.

\noindent\textbf{What area of the paper need improvement?}

The paper assumes that the number of tasks per job is a fixed parameter k, not allowing the number of tasks per job to vary from parallel job to parallel job. The paper considers a specific form of zero queueing delay which allows tasks in a job to wait in queues for non-negligible amounts of time. The paper assumes Poisson arrives and exponential service, with the hope to extend the results to general service time distributions.


\noindent\textbf{Other comments for author}

The paper assumes that the number of tasks per job is a fixed parameter k. It would be interesting to extend the analysis to consider the number of tasks per job k to be sampled from a probability distribution with a given mean $\bar{k}$, and attempt to show that the established results in terms of k then hold in an appropriate sense with respect to the mean number of jobs $\bar{k}$.

{\color{blue}\noindent\textbf{Response.}
This is a very interesting proposal.  We believe that if $k$ follows a distribution with a finite support set $\{k_{\ell},k_{\ell}+1,\cdots,k_r\}$ such that $k_r \leq k_{\ell}^c$ where $c$ is a positive constant, the achievability results should still hold.  But this is a question that needs much more scrutiny and we will pursue it in future work.
}



The paper considers a specific form of zero queueing delay that actually allows tasks in a job to wait in queues for non-negligible amounts of time. The paper should mention other possible forms of zero queueing delay that are more stringent, and discuss how the analysis presented in the paper might be extended to address these more stringent forms of zero queueing delay.

{\color{blue}\noindent\textbf{Response.}
We thank the reviewer for this great suggestion!  We have added Section~6 to discuss the more stringent notion.  Please refer to our responses to one-shot revision requirements (I.d) and (I.e).
}

In section 2, there is no need to repeat the expression for the specific form of zero queueing delay. Simply make reference to equation (1) instead.

{\color{blue}\noindent\textbf{Response.}
We have made a reference to equation (1).  But we do have a slight preference to keep the expression since we wanted the model section to be relatively self-contained.  We have changed it from on display to in line to minimize the space needed.  Please see Page~6. 
}

Punctuation is missing after some of the equations. E.g., equation (13).

{\color{blue}\noindent\textbf{Response.}
Fixed.  Please see equation (14) on Page~11.
}



==> simulation-old.tex <==
% simulation results when scale up N
% figure: x-axis: N
% y axis: delay/max{task delays}
% curves: different d's
% address the comment that zero queueing delay can be achieved with reasonable values of k and N
% explore the threshold of d for zero queueing delay

% comparison with non-parallel setting

{\color{blue}
In this section, we perform three sets of simulations to demonstrate our theoretical results and explore settings beyond those in our theoretical analysis.  The first set illustrates the scaling behavior of the system as $N$ grows under various probe ratios, and investigates the gap between our achievability results and impossibility results.  The second set looks into the effect of parallelization by comparing our setting with a setting where the tasks of a job cannot be executed in parallel. Finally, the third set experiments on more general service time distributions beyond the exponential distribution.


\subsection{Scaling Behavior with Various Probe Ratios}\label{subsec:scaling}
This set of simulations use the setting of our theoretical results with $\lambda=1-N^{-0.3}$ ($\alpha=0.3$ and $\beta=1$). We let $k$, the number of tasks per job, scale with $N$ as $k = \lfloor \ln^2 N \rfloor$.  The values for $N$ and the corresponding $k$ used in the simulations are given in Table~\ref{table:scale-system}. These values are reasonable in practice considering that datacenters nowadays typically have tens of thousands of nodes (each with multiple cores) per cluster and a job may consist of hundreds of tasks \cite{amvrosiadis_2018}.

%In this simulation, we follow the setting of our basic model. Jobs arrive in a Poisson process with arrival rate $ \frac{N(1-N^{-0.3})}{k}$, so $\alpha = 0.3$ here. Each job contains $k$ parallel sub-tasks whose service time independently follows a  exponential distribution with mean $1$. Jobs are scheduled using batch-filling algorithm. Twelve scales of systems are considered as per Table \ref{table:scale-system} where $k = \lfloor \ln^2 N \rfloor.$
% \begin{table}[!hbp]
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% $N$ & 32   & 64   & 128  & 256   & 512   & 1024  \\ \hline
% $k$ & 12   & 17   & 23   & 30    & 38    & 48    \\ \hline
% $N$ & 2048 & 4096 & 8192 & 16384 & 32768 & 65536 \\ \hline
% $k$ & 58   & 69   & 81   & 94    & 108   & 122   \\ \hline
% \end{tabular}
% \caption{Scaling of the System}
% \label{table:scale-system}
% \end{table}
\begin{figure}[!hbp]
\begin{minipage}[c]{.4\textwidth}
\centering
\begin{tabular}{r r r r r}
\\
\toprule
$N$ & 32   & 64   & 128  & 256   \\
$k$ & 12   & 17   & 23   & 30    \\
\midrule
$N$ & 512   & 1024  & 2048 & 4096 \\
$k$ & 38    & 48    & 58   & 69 \\
\midrule
$N$  & 8192 & 16384 & 32768 & 65536 \\
$k$  & 81   & 94    & 108   & 122   \\
\bottomrule\\
\end{tabular}
\captionof{table}{Scaling parameters.}
\label{table:scale-system}
\end{minipage}
\hspace{0.3in}
\begin{minipage}[c]{.5\textwidth}
\centering
\scalebox{0.32}{\input{picture/diff-d.pgf}}
\vspace{-0.1in}
\caption{Queueing delays under different probe ratios: $d_1$ is sufficient for convergence to zero queueing delay; $d_1>d_4>d_3>d_2$.}
\label{fig:different-d}
\end{minipage}
\vspace{-0.2in}
\end{figure}


We explore four scaling settings of the probe ratio.  The first setting uses a probe ratio of $d_1 = \frac{4}{(1-\lambda)h}=\frac{4N^{\alpha}}{h}$ with $h = \lceil\frac{\log k}{\log \log k} \rceil$, which satisfies the conditions in Theorems~\ref{main_theorem_1} and \ref{theorem zero delay} to achieve zero queueing delay.  The second setting uses a probe ratio of $d_2 = \exp{(0.5\log N / \log k)}$, which is slightly larger than the value in Theorems~\ref{main_theorem_2} and \ref{theorem lower d} that guarantees non-zero queueing delay.  The other two settings use probe ratio values $d_3$ and $d_4$ that interpolate between $d_1$ and $d_2$ to investigate the threshold under which the system transits from zero queueing delay to non-zero queueing delay.  Note that $d_1>d_4>d_3>d_2$ for all values of $N$ in the simulations. More details of the settings can be found in Appendix~\ref{sec:experiment}.

Figure~\ref{fig:different-d} shows the simulation results for the queueing delay $\frac{\expect[T-T^*]}{\expect[T^*]}$.  The curve for $d_1$ demonstrates the trend for the queueing delay to converge to zero as predicted by the theoretical results.  It does not exactly reach zero but becomes reasonably close. Under the probe ratios $d_2$ and $d_3$, the queueing delay clearly deviates from zero.  Under the probe ratio $d_4$, the queueing delay flattens out after some initial drop as $N$ becomes large.  Therefore, it is plausible that the transition from zero queueing delay to non-zero queueing delay happens at a probe ratio value near $d_4$.  Since $d_4$ is much closer to $d_1$ than to $d_2$, we expect our impossibility results to be not tight.  Pinning down the exact threshold for the transition (or proving the nonexistence of such a threshold) is of great theoretical interest and we leave it for future research.

%Let $h = \lceil\frac{\log k}{\log \log k} \rceil$. We set $d_1 = \frac{4}{(1-\lambda)h},d_2 = e^{0.5\log N / \log K}$ as per Theorem \ref{theorem zero delay} and Theorem \ref{theorem lower d}. Besides, two other scalings of the probe ratio, $d_3 = d_2 + \sqrt{d_1}$ and $d_4 = d_2 + d_1^{7/8}$, are studied for a sharper threshold to achieve zero queueing delay. We refer the reader to Appendix \ref{sec:experiment} for a detailed setting. The value of $\frac{\expect[T]}{\expect[T^*]}$ , which we call relative job delays, is shown in Figure \ref{fig:different-d}.
% \begin{figure}
% \begin{minipage}[t]{.45\textwidth}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% $N$ & 32   & 64   & 128  & 256   \\ \hline
% $k$ & 12   & 17   & 23   & 30    \\ \hline
% $N$ & 512   & 1024  & 2048 & 4096 \\ \hline
% $k$ & 38    & 48    & 58   & 69 \\ \hline
% $N$  & 8192 & 16384 & 32768 & 65536 \\ \hline
% $k$  & 81   & 94    & 108   & 122   \\ \hline
% \end{tabular}
% \captionof{table}{Scaling of the system}
% \label{table:scale-system}
% \end{minipage}
% \hspace{0.3in}
% \begin{minipage}[t]{.45\textwidth}
% \centering
% \scalebox{0.32}{\input{picture/diff-d.pgf}}
% \caption{Relative job delays under different probe ratios. Here $d_1$ is the proved sufficient probe ratio to achieve zero queueing delay; $d_2$ is the proved necessary probe ratio; $d_3,d_4$ are two intermediate probe ratios.}
% \label{fig:different-d}
% \end{minipage}
% \end{figure}
%Figure \ref{fig:different-d} verifies our theory that the probe ratio $d_1$ leads to asymptotic zero queueing delay while the probe ratio $d_2$ always results in non-negligible delays. However, Figure \ref{fig:different-d} also indicates that the sharp lower bound may indeed be close to the upper bound $d_1$, which we leave for future research.  


\subsection{Effect of Parallelization}
This set of simulations demonstrates how parallelization plays a critical role in reducing the probe overhead needed for achieving zero queueing delay.  Towards this end, we simulate a system where the parallel structure of jobs is taken away.  In particular, each job in this non-parallel model is indivisible with an exponentially distributed service time with mean equal to $k$ (denoted as $\text{Exp}(1/k)$). The queueing delay for such non-parallel jobs is defined with respect to $T^*\sim\text{Exp}(1/k)$, which is the job delay without queueing.  Figure~\ref{fig:non-parallel} shows that the probe overhead that yields zero queueing delay for parallel jobs is no longer sufficient for achieving zero queueing delay for such non-parallel jobs.
% needs to confirm probe overhead

%We next compare our result with the non-parallel setting. To be specific, this simulation follows the same setting as in the last one. But in addition to parallel jobs, we consider non-parallel jobs where each job only contains one task whose service time is exponentially distributed with mean $k$. Then every parallel and non-parallel job shares the same expected total amount of work equal to $k$. To study the benefit of a parallel structure, we compare the relative delays of parallel and non-parallel jobs using the same probe ratio $d_1$. Results are shown in Figure \ref{fig:non-parallel}.
\begin{figure}
\begin{minipage}[t]{.45\textwidth}
    \centering
    \scalebox{0.32}{\input{picture/nonparallel-comparison.pgf}}
    \vspace{-0.1in}
    \caption{Effect of parallelization on queueing delays.}
\label{fig:non-parallel}
\end{minipage}
\hspace{0.3in}
\begin{minipage}[t]{.45\textwidth}
    \centering
    \scalebox{0.32}{\input{picture/diff-dist.pgf}}
    \vspace{-0.1in}
    \caption{Queueing delays under different service time distributions.}
    \label{fig:different-dist}
\end{minipage}
\vspace{-0.2in}
\end{figure}

\subsection{More General Distributions for Task Service Times}
The last set of simulations explore distributions beyond the exponential distribution for task service times.  Figure~\ref{fig:different-dist} shows the results for three distributions: (1) \emph{Exponential distribution} with rate $1$ ($\text{Exp}(1)$).  This is the baseline distribution that is assumed for our theoretical analysis. (2) \emph{Bounded Pareto} in range $[1,1000]$ with a shape constant $1.5$. (3) \emph{Hyper-exponential} that follows $\text{Exp}(1)$ with probability $0.99$ and $\text{Exp}(0.01)$ with probability $0.01$.  We re-scale the arrival rates so all the systems have the same load $\lambda=1-N^{-0.3}$.  The probe overhead is chosen to be the $d_1$ in Section~\ref{subsec:scaling} such that zero queueing delay is provably achievable under the exponential distribution. 

We observe that empirically, the queueing delay has a trend that approaches zero under all the three distributions, although the latter two distributions have larger coefficients of variation than the exponential.  These simulation results suggest that our theoretical results have some robustness with respect to service time distributions.  We comment that there is little existing work on zero queueing delay for general service time distributions with the exception of \cite{b5}, which studies the Coxian-2 distribution for non-parallel jobs.  Generalizing our analysis to general service time distributions is a research direction that deserves much further effort, as it is for many problems in queueing systems.


%The last simulation generalizes the parallel-job model to different service time distributions for tasks. Denote the service time of a task by $S$. In particular, we consider the following three distributions: 1) \textbf{Exp(1)}, the service time follows a exponential distribution with mean $1$; 2) \textbf{Bounded Pareto}, the task service time $S$ is sampled from a bounded Pareto distribution in range $[1,1000]$ with the shape constant $1.5$; 3) \textbf{Hyper-exponential}, the service time $S$ follows Exp(1) with probability $0.99$, and follows Exp(0.01) with probability $0.01$. Note that in the simulation, the arrival rate of jobs is set as $\frac{N(1-N^{-0.3})}{k\expect[S]}.$ To study the effect of service time distribution, we fix the probe ratio as $d_1$ for all three distributions. Figure \ref{fig:different-dist} then shows how the convergence of relative delays is related to the service time distribution.

%For both the hyper-exponential distribution and the bounded Pareto distribution, our reduced probe ratio is feasible to (asymptotically) achieve zero queueing delay.
}

